Learning Alternative Ways of Performing a Task

A common way of learning to perform a task is to observe how it is carried out by experts. However, it is well known that for most tasks there is no unique way to perform them. This is especially noticeable the more complex the task is because factors such as the skill or the know-how of the expert may well affect the way she solves the task. In addition, learning from experts also suffers of having a small set of training examples generally coming from several experts (since experts are usually a limited and expensive resource), being all of them positive examples (i.e. examples that represent successful executions of the task). Traditional machine learning techniques are not useful in such scenarios, as they require extensive training data. Starting from very few executions of the task presented as activity sequences, we introduce a novel inductive approach for learning multiple models, with each one representing an alternative strategy of performing a task. By an iterative process based on generalisation and specialisation, we learn the underlying patterns that capture the different styles of performing a task exhibited by the examples. We illustrate our approach on two common activity recognition tasks: a surgical skills training task and a cooking domain. We evaluate the inferred models with respect to two metrics that measure how well the models represent the examples and capture the different forms of executing a task showed by the examples. We compare our results with the traditional process mining approach and show that a small set of meaningful examples is enough to obtain patterns that capture the different strategies that are followed to solve the tasks.

==> sections/background.tex <==
\section{Background} \label{background}
%\textcolor{red}{Si vamos a enviarlo al ESWA no podemos tirarnos directamente al río del Surgical Training, tenemos que enfocarlo primero a supervisión y cómo se hace para después sacar la parte de Surgical trainig como ejemplo de aplicación de lo que se va a desarrollar. Vamos, primero un Background en Supervision y después nos metemos con Surgical Training.}

% \todo[inline, color=green!40]{
% Outline: 
% - Supervision de actividades \\
% 	\tab- Distinción de actividades simples (visión por ordenador y DL) y complejas (data-driven approa./ knowledge-driven approa.)\\
%     \tab- Sistemas de supervision usando la separación de arriba.\\
% 	\tab- Introducir el sistema supervasion como knowledge-driven approa.\\
% - Reconocimiento de planes \\
% 	\tab- Modelización de workflow a mano \\
%     \tab- Modelización de workflow por librerías de planes \\
%     \tab- Alternativa -> Aprender workflow a partir de ejemplos de planes\\
%     \tab- Presentación de nuestra propuesta de este artículo\\
%     \tab- Presentación del dominio sobre el que hemos construido nuestra approa. y los problemas que presenta (pocos ejemplos y diversidad de formas).
% }

% For related work
% References:
%	- Get from introduction [Yan,2005] 
%	- Graph aggregation
%	 	- Yan, 2005 
%			- SPLAT algorithm
%		- Hu, 2005
%			- CODENSE system
% 	- graph matching applications (by domains):
%		- Web 
%			- user navigation
%			- web crawlers (page rank paper)
%		- genetics 
%			- graph papers which use mutag dataset
%		- Image processing 
%			- Get from related work [Yan,2005]
%	- Surgical process analysis using graphs
% 		- Schumann 
%	- Graph similarity measures 
% 		- [Koutra, 2011] 
%		- GED
%			- GEDEVO system
%			- [Cao, 2013]
%		- from graphkernels
%			- Histograms
%			- Gaussian Histogram
%			- Graphlet papers
%			- Weisfeiler-Lehman Kernel
%			- Shortest path and random walks
%		- Other measures
%			- Eigenvalue
%			- [Papadimitriou, 2010] (Some of these metrics are shared with DELTACON paper [Koutra, 2013])
%				- Vertex/Edge Overlap (VEO) (Jaccard index)
%				- Vertex ranking (VR)
%				- Vertex/edge vector similarity (VS)
%				- Sequence similarity (SeqS)
%				- Signature similarity (SS) 
%			- [Koutra, 2013]
%			- Probabilistic measures


% Reconocimiento de actividades simples

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

 
% New trends in automatic supervision 

% Computer vision-based supervision systems have benefited FROM the recent developments in the Activity Recognition (AR).

% Strauch, B. (2017). Investigating human error: Incidents, accidents, and complex systems. CRC Press.

% Ambient Assisted Living (AAL) [1] denotes concepts,
% products, and services that interlink and improve new
% technologies and social systems, with the aim of enhancing the
% quality of life for all people during all stages of their lives.
% AAL could therefore be translated best as intelligent systems of
% assistance for a better and safer life [6]. The potential range of
% services belonging to the AAL domain is huge. It encompasses
% any assistive service that facilitates daily life. The classification
% scheme [7] shown in Figure 1 structures this domain into six
% stereotypical subdomains with clearly separated responsibilities.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\sidenoteMJ{No se si despues de   la seccion de discusion pega esta de trabajo relacionado. Ni siquiera creo que haga falta añadir esta seccion o si se podría mover mucho mas simplificada a despues de la intro}
\sidenoteCM{Como ya comentamos, yo pasaría algunas referencias a la introducción y eliminaría esta sección} 
\subsection{Automatic supervision of human activities}
\sidenoteMJ{este apartado esta muy orientado a supervision que creo ya no toca. Yo extraería la parte de activity recognition unicamente}
% Reconocimiento de actividades básicas
% Reconocimiento de actividades complejas usando data-driven approaches y knowledge-driven approaches
The recognition of complex human activities has been widely addressed by the area of Activity Recognition (AR). AR can be considered the base of the most of supervision systems. In AR, a distinction can be made between data-driven approaches and knowledge-driven approaches following the differentiation provided in \citep{chen2012sensor}. Data-driven approaches (\citep{hoey2010automated}, \citep{sanchez2008activity}, \citep{patterson2005fine}, \citep{kruger2014computational}) are characterised by using supervised (e.g., Hidden Markov Models (HMM), Linear Dynamical Systems (LDSs)) and unsupervised (e.g., KNN) machine learning techniques to address the problem. These are powerful tools when facing uncertainty and temporal information but they require large datasets for learning the activities. This dependency of data makes data-driven approaches to be sensitive to issues such as data scarcity or even the ``cold start'' problem: the problem that emerges when a data-driven application does not have the minimum amount of data to learn the task and operate. In addition, limitations in scalability and reusability may arise here due to difficulties in applying the learnt activity models from one person to another. Above all, despite being possible to describe a scene by recognising the sequence of actions, in many cases, it is meaningless for understanding the task by itself, so a high-level reasoning is required to those effects. 

By contrast, knowledge-driven approaches (\citep{okeyo2011ontology}, \citep{ye2015usmart}, \citep{chen2012knowledge}, \citep{chen2008logical}, \citep{bouchard2006smart}) are characterised by their reusability, semantic clarity and a lower dependency from the training data. Activity models consist of rules that define the logic of the task and its constraints. This representation make it possible the introduction of domain knowledge about tasks to supervise. This prior knowledge can be translated easily into reusable structures, i.e., schemes, logical representation or ontologies, which are then used for reasoning about the relationships between activities, objects, temporal and spatial context. Furthermore, they provide some interesting features, such as deduction, induction, and abduction, that pave the way for the generation of new knowledge from examples or predicting future events using commonsense reasoning. On the other hand, knowledge-driven activity modelling has limitations when handling noisy and uncertain data from sensor readings, as well as managing temporal information. In some cases, these models could be viewed as quite rigid and incomplete \citep{chen2012sensor}. 

% Sobre sistemas de supervision
The applicability of both types of approaches inside a real automatic supervision system has become a hot topic in recent years. On the side of data-based systems, we can find that Markov-based models are predominant. For instance, in \cite{hoey2010automated} the authors present a data-driven system for assisting persons with dementia during handwashing. The process is modelled by using a \textit{partially observable Markov decision process} (POMDP). This type of model makes it possible to represent the uncertainty control and the user’s mental states by adding rewards and costs to the actions. The results showed that the system is accurate and provides reliable assistance to people with dementia. Kitchen activities supervision is also a hot topic for data-driven approaches. \cite{kruger2014computational} studied the feasibility of Computational Causal Behaviour Models (CCBM) for providing assistance when the user is cooking the meal. By distributing a realistic sensor setups on the kitchen objects and the human subject (using wearable inertial measurement units or IMUs), the CCBM is not only capable of recognising the current cooking activities, but also the user intentions and goals from noisy sensor data. The topic of supervising cooking tasks through a data-driven approach has also been addressed by \cite{yordanova2017s}, \cite{rohrbach2012database}, and  \cite{neumann2017kognichef}. A wider scope would include also supervision in a whole smart environment using sensor data \citep{twomey2016sphere}, \citep{intille2006using}, \citep{krose2008care}, \citep{crandall2011tracking}.

% Knowledge-based approach: \citep{yordanova2017situation}
Alternatively to data-based supervision systems, the knowledge-based systems try to take full advantage of other knowledge resources in contexts where accessing training data is complicated. These resources may be the use of ontologies, textual descriptions of the task or specific background knowledge. For instances, in \cite{okeyo2011ontology}, \cite{ye2015usmart} \cite{chen2012knowledge} different knowledge-driven approaches are proposed to recognise the behaviours of smart home inhabitants using ontologies. Other systems try to take advantages from reasoning about the behaviour of the person in the environment in order to prevent situations of risk. \cite{chen2008logical} presents a knowledge-driven framework for Smart Homes based on the Event Calculus (EC) formalism \citep{mueller2014commonsense}. Specifically, they model both sensors activation and objects properties with EC events and fluents, respectively. By using features of the commonsense reasoning, the system is capable of reasoning about inhabitant behaviour and foresee events of risk derived from the human interaction with the environment. A similar idea can be found in \cite{bouchard2006smart}, where the lattice theory and action description logic is used to recognise the inhabitant plans and reason about them in order to prevent home accidents of people how to suffer from cognitive impairments (e.g., Alzheimer). Although the current knowledge-based systems are powerful when performing supervision in contexts with a few examples, they do not address the topic of learning from some demonstrative examples of a task in order to complete or extend the prior knowledge. 

% Sobre el sistema SUPERVASION
The authors of the present paper have established the basis for a knowledge-based supervision system that addresses this issue \citep{monserrat2016knowledge}. The purpose of this automatic supervisor is to assist humans when they are learning or performing complex tasks. Unlike the previous approaches, the innovative idea is that the system learns any procedure from some background knowledge and one (or a few) meaningful observations by using an ``Induction by Abduction'' process. Then, it can trace the steps and spot the deviations of operators performing that task afterwards. When the number of examples is constrained by the domain, this problem is only feasible with a strong bias. Here, this bias is represented by the domain knowledge provided by experts, which must be introduced initially as a high-level textual description \citep{yordanova2017knowledge}, and then enriched incrementally by the system in accordance with several low-level demonstrations of how that task must be done in practice \citep{nieves2017low}. Specifically, and as a result of each demonstration, a sequence of activities can be inferred from the detected events, such as the tool actions and movements. In this paper we address the question of how to generalise about multiple demonstrations, when there can be multiple ways of solving the task and this task demands a high level of human dexterity (i.e., more activities than are strictly necessary, appearance of peculiar forms or \textit{styles} of solving the task, etc). In short, the search for the general process, together with its possible variations, which underlies these demonstrations.

\subsection{Process modelling}
The issue of determining the process behind a human task has been addressed in many ways. The first possible approach is to create an activity model manually. This consists of defining the set of activities that are required and establishing the correct flows of steps from the start activity to the final activity of the task. This type of approach requires time and effort since the model must be defined and the conditions of each step must be programmed. It also ends up being very subjective, because, in many cases, ``what should be'' is programmed rather than how the task is actually carried out in practice. A simple way to save this effort is to create a completely connected model and then learn the transitions from a set of training runs. Probabilistic models are often used, such as Hidden Markov Models (HMMs) \citep{boger2005decision}, \citep{kalra2013detection}, \citep{duong2009efficient} or Dynamic and Naïve Bayes networks \citep{baker2009action}, \citep{dai2008group}, \citep{oh2014probabilistic}, where transition probabilities are learned. This method is better adapted to the real behaviour of the process since it is based on evidence, but it has limitations. The most obvious is that when the complexity of the task increases, the model can end up in an explosion of possible states due to all the combinations that are made \citep{sadilek2012location} \citep{rosen2002task}. On the other hand, this type of model also suffers from the problem of "cold start" and usually require a large amount of data \textcolor{blue}{to perform accurate supervision \citep{chen2012sensor}}\sidenoteMJ{lo de supervision?}.

In the area of Plan Recognition \citep{sukthankar2014plan}, the creation of the process model based on the definition of scripts is proposed as a solution. These scripts allow you to establish the preconditions and effects that activities have on the environment to be monitored \citep{kruger2012towards}. Later, these scripts are compiled creating a probabilistic model with the space of possible states that allow the conditions established in the scripts. In a second phase, the model is trained to learn the probabilities of transition of the task as in the case of a completely connected model. The biggest limitation comes from having to define the scripts manually, in addition to the already mentioned "cold start" and the need for training data. To facilitate this task of manually defining the scripts, methods have been proposed in the literature to infer preconditions and effects from other available resources such as a description of the task in natural language \citep{yordanova2017texttohbm}. Nevertheless, it can not completely avoid manual adjustment of the model.

A different approach is to infer the process model directly from observing demonstrative examples. We can find two areas that address this challenge from two different perspectives: imitation learning \citep{hussein2017imitation} and process mining \citep{van2016process}. In the first one, the objective is that a machine (robotics in many cases) can learn the necessary movements (i.e., policy) to solve a simple task through examples that show how to do it. In these cases, the figure of the human expert appears who is in charge of making the examples while the machine observes it. The current trend in imitation learning focuses on the use of deep learning techniques \citep{xu2018neural}\citep{duan2017one} \citep{finn2017one}. Although they have given surprising results even in scenarios with few examples, the tasks they are able to learn and solve are still very basic (e.g., stacking boxes). In addition, the fact of using deep learning hinders the traceability and analysis of the knowledge acquired by the system. On the other hand, the approach proposed by process mining is different. As in imitation learning, its objective is to learn a model of a process from the observation of various executions of it. The main difference with deep learning methods (black box models), is that the techniques proposed in process mining are based entirely on algorithms that allow traceability and analysis of the entire process of generalisation, from the sequences to the final model obtained. In turn, the proposed models are easily interpretable by non-expert people, being also easily processable to obtain other representations (e.g., logic rules). This last approach is the basis of the algorithms proposed in this paper.\sidenoteMJ{falta algo que nos diferencie de process mining}


%%%%%%% Versión antigua %%%%%%%%%
% Reconocimiento de planes y plan synthesis
%The issue of determining whether the observed activities can be interpreted as part of a predefined process has been widely addressed by the areas of Plan Recognition (\citep{sukthankar2014plan}) and Process Modelling \citep{van2016process}. In Plan Recognition literature (\cite{kruger2016activity}, \cite{jachowicz1997describing} and \cite{garland2002continuous}), a plan is defined as a sequence of actions starting from an initial state to a goal state, where one assumes that user actively tries to achieve the goal. Plan Recognition poses several challenges to be addressed for modelling plans in a computerised manner. For instance, a traditional way to face the task representation and reasoning is by creating a stochastic activity model. Firstly, task steps are defined as possible sequences of activities which fulfil the task by connecting the initial and final states in the representation. Then, a training phase is applied for learning the predominant ways from observed data. During the task supervision, the current state is inferred from observed data and user’s potential future actions and the possible goals are reasoned from there. These models are usually based on supervised machine learning techniques such as Hidden Markov Models (HMMs) (\cite{boger2005decision}, \cite{kalra2013detection}, \cite{duong2009efficient}) and dynamic and naïve Bayes networks (\cite{baker2009action}, \cite{dai2008group}, \cite{oh2014probabilistic}). 

%Even though these approaches have demonstrated their utility on countless occasions in task automation, there are several drawbacks when it is used in automatic supervision in complex environments. First of all, there are applied a careful handcrafting to model the scenario to be supervised. This fact may suppose an important drawback when task complexity grows up by its possible intermediate state combinations. One way to semi-automate this process is by defining plan libraries, where the causal semantics of human actions are depicted there as preconditions and effects rules. Those libraries are processed in a further step to deploy all possible ways of fulfilling a task which forms the computational state space. However, the exact representation of all possible states in continuous scenarios is not feasible due to the lack of memory. Nevertheless, approximate methods have been proposed in recent years \citep{kruger2014computational}. Both approaches, manual modelling and the definition of libraries, involve an unnecessary waste of time and human labour effort and tend to be biased by what “may” be done afterwards rather than modelling ``on the fly'' from observed events that took place. Furthermore, they still require large datasets for training, which makes its application difficult in domains with few examples. As a result, these approaches are limited in terms of versatility, reusability and knowledge generalisation. %Moreover, for some supervision scenarios, unfolding all possible transitions between actions could be overstated because many of the states do not represent the right way to proceed. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This transformation allows use of AI planning, in particular, the use of planners capable of finding a plan set.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%An alternative method lies in learning the plausible states from a set of ``rich'' process executions (\cite{winner2002analyzing}, \cite{blythe2001integrated}, \cite{benson1995inductive} and \cite{wang1995learning}). In \cite{yang2005learning}), and later in \cite{yang2007learning}, the authors proposed an algorithm to construct the state information from several execution examples of the same process. Each execution is formed by a sequence of parametrised activities together with the initial states and the goals conditions. From this incomplete knowledge, their approach automatically guesses a minimal logical action model that can explain most of the provided examples. This inductive process goes from the specific to the general, where a system (i.e., learner) generalises the observations and infers a general theory (pattern, hypothesis or model) that explain them. One of the main problems of the approaches based on inductive inference is how to efficiently organise the search of the solution in the hypothesis space. In that context Inductive Logic Programming (ILP) \cite{muggleton2012ilp} appears to be one of the best tools to perform that task. In contrast to other inductive paradigms, in ILP there are positive and negative observations about the concept to be learnt. Both kinds of evidences are used by the ILP systems to decide when to generalise/specialise the current hypothesis as well as to define the stopping criterion that indicates that a solution has been found. 
%Among the ILP systems %\cite{lavrac1994inductive},
%we can cite GOLEM%\cite{muggleton1990efficient}
%, MARVIN %\cite{sammut1986learning}
%or CIGOL %\cite{muggleton1988machine} 
%as typical examples with a bottom-up search, whereas FOIL%\cite{quinlan1990learning}
%, FOCL %\cite{pazzani1992utility} 
%or MARKUS %\cite{grobelnik1992markus} 
%systems use a top-down search.

%Similar generalisation mechanism can be found in our approach. 
%Similar to ILP, we present in this paper an inductive top-down approach to learn models of processes from a little number of correct expert executions. As has been stated, this implies that those models must be learnt from a few positive examples and without negative ones. Besides, the learning process must consider all de process execution as a whole avoiding local decisions to obtain coherent results and must be able to detect the different ways of executing the process. In this context, it seems that Process Mining \cite{van2016process} combined with ILP techniques are ideal to address the mentioned process modelling. Process mining is a family of techniques in the field of process management that support the analysis of business processes based on event logs. Two of its applications are in process discovery and conformance checking. The first one can be used to learn process models from traces of activities (i.e., real process executions or \textit{event log}) and the second one can be used to evaluate the agreement between the learnt model and the observed examples, or possibly new ones, with different quality metrics. In a similar manner than process mining does, we propose an approach that use observations of a task to infer the underlying process models that represent it. However, the previous techniques cannot be applied directly for supervision because of the presence of non-essential activities and the diversity of the ways of performing a process. In order to avoid these limitations, we have used Dependency Graphs (from process mining techniques) to represent the process examples and applied graph theory and ILP techniques to obtain the process models from those examples. 

%We have contextualised our proposal in extracting process models from a common suturing task from surgical training domain. This is a highly complex task where some skilled surgeons develop a particular manner to undertake some surgical procedures. Therefore, it is likely that two sequences of activities, maybe from two different surgeons, be perfectly valid, being one significantly different to the other. Several data-driven approaches have tried to learn those tasks by using Markovian structures and low-level motion data \cite{varadarajan2009data} \cite{tao2012sparse} \cite{lin2005automatic} \cite{reiley2008automatic}, being penalised by the previous facts as shown the results of \cite{ahmidi2017dataset}. Therefore, it converts the aforementioned context into the ideal framework in which to check our developments. 



==> sections/introduction.tex <==
\section{Introduction} 

%In this paper, we propose a new method based on Process Mining and Inductive Programming to learn process models for posterior applications in automatic supervision systems. 
Nowadays, there are multiple fields of research that are investigating automatic systems that monitor, recognise and respond to human behaviours, such as Ambient Intelligent \citep{camacho2014ontology} And Context-aware systems \citep{hong2009context}, Advanced Driving Assistants \citep{vskrjanc2018evolving} or Surveillance systems \citep{kardas2017svas} \citep{mabrouk2018abnormal}. In fact, the potential of an automatic supervision system of monotonous and/or complex human processes could be a reasonable alternative to their automation, making the human performance more reliable and efficient because of the constant monitoring at a considerably reduced cost. This supervision would care about whether the operators would be developing the process correctly, detecting deviations from the established models of the process, and advising them in real-time because deviations of the model or by suggesting activities to accomplish the goals of the process (meaningful feedback). As a result, an automatic supervisor could prevent some processes from suboptimal results or implying a potential risk due to human mistakes \citep{birkmeyer2013surgical}. 

In order to do all this, the supervision system need to learn the essence of how one process should be done, coded by a programmer or learnt automatically from examples and procedures provided by experts. Manual coding is time-consuming, rigid and prone to obsolescence. Besides, it requires a big effort to define, or in the extreme case, to directly program all the possible models of performing a process, as well as updating them when new models appear over time. On the other hand, a real automatic supervisor must be general, transversal and pervasive enough to be tuned to multiple domains. Moreover, the number of available examples is often limited, but still the system must learn the different ways in which a process can be performed toward carry out correct supervision. 

Traditionally, similar learning processes have been addressed in Activity Recognition (AR) \citep{sukthankar2014plan}, using both data-based approaches and knowledge-based approaches \citep{chen2012sensor}. To date, data-based approaches have been the predominant way to generalise task models, relying on intensive use of pre-existent data from users’ activities. However, these approaches are not suitable for domains where there is not enough data. Besides, in some cases, it is necessary to define the structure of the task to be learnt previously \citep{hoey2010automated}. An alternative way (i.e., knowledge-based approaches) implies to take advantage of the previous knowledge (bias) about the domain as a resource to generalise or learn a procedure. For example, logic-based approaches obtain semantically clear and compact models, but have problems adapting to different users’ activity habits and handling examples with noise (i.e., infrequent behaviours).

In this paper, we aim to provide a generalisation method to automate the extraction of the essential workflows (i.e., process models) from a few expert executions. Our method overcomes the limitations of the data-based (i.e., learn from a few examples) and knowledge-based approaches (i.e., different behaviours, different models), by using a method based on process mining techniques \citep{van2016process}, Inductive Programming and graph theory. As a result, we obtain models in the form of dependency graphs (\citep{van2004workflow}, \citep{yan2005mining}, \citep{carrington2005models}, \citep {papadimitriou2010web}), typical representation for process models where the model nodes represent the involved activities, and the directed arcs represent the order relation between these activities. These models have two advantages: they are easily understandable and make it possible to filter the non-essential activities \citep{van2016process}. One activity is considered non-essential if its execution is not necessary to finish the process correctly. The algorithm also ensures the validity of each model, as a complete representation of the process, and the feasibility of it by checking that, at least, one training example is covered by the output model. Finally, we have analysed the generalisation, simplicity and fitness properties of the resulting models. As far as we know this is the first approach that proposes the combination of dependency graphs and an inductive method for process modelling in a knowledge-based supervision system. To analyse the applicability of the model, we have tested the potentiality of this method in a very challenging environment that considers all the mentioned requirements: the automatic skill supervision in surgical training tasks.

The rest of this paper is organised in the following manner. Section \ref{motivation} presents briefly the motivation of this work. In this section we want to answer the question of why we have developed this research. Section \ref{matandmet} presents our mining approach based on dependency graphs. Then, Section \ref{s:results} presents the experimental setup and the results of applying our approach with a set of real examples of a surgical exercises. In Section \ref{s:discussion} we discuss the experimental results and the strengths and limitations of our method. Section \ref{background} reviews the literature on automatic supervision and process modelling. Finally, Section \ref{s:conclusions} outlines our conclusions and further research directions.

%%%%%%%%%%%% Versión antigua con Comentarios Jose %%%%%%%%%%%%

% Today, there are many human tasks whose automation is not possible yet, despite being repetitive. The automatic supervision of these tasks has arisen as a suitable step for making them more reliable and efficient, in the interim of making them fully automated. Also, supervision and overseeing may be key for contexts where other automated systems are being used, but still not very reliable. 
% %Despite the human interaction is still indispensable to perform such tasks, a  system could assist the human in the development of the task. In this sense, that system, as 
% An automated supervisor would be able to monitor whether operators are performing the task correctly, detect deviations from the established plans, and advice them in real time %, if that were the case, 
% with meaningful feedback. \sidenoteJose{A partir de aqui se repite lo mismo una y otra vez. Reescribo}Automated supervision could have a significant effect on two important spheres. On one hand, some tasks may be easily spoilt, may lead to suboptimal results or imply a potential risk by a human mistake. The supervisor system could trace the operator activities and spot the deviations from the expected performance, %. The same applies to those jobs subject to pre-established 
% workflow or protocol. %, where automated supervision would make it more secure. 
% On the other hand, humans learn some tasks more efficiently if they have continuous supervision and get meaningful feedback, but this overseeing (from an expert or a teacher) is usually expensive. Hence, the acquisition of new skills in training environments would be enhanced through systems performing automated supervision and useful feedback. Indeed, poor technical skills have been associated with adverse outcomes or even tragic consequences \cite{birkmeyer2013surgical}. These two stages (training and operation) are directly connected. The better training is through intensive monitoring and feedback the less prone to errors the operators will be. This has been shown % at is why in some domains such as surgery, it is foreseen that those systems can be potentially beneficial to improve the  
% in surgical/interventional care \cite{vedula2017surgical}.  \sidenoteJose{De nuevo nos repetimos un montón en lo que queda.} In some educational contexts, the traditional model of teaching skills relies on supervision and demonstration by experts in the matter.This method has traditionally suffered important limitations, such as limited access to realistic test beds or the availability of experts’ time to give immediate feedback and guidance during each exercise. Automatic supervisors, as coaching systems, would be an alternative to enable inexperienced trainees to learn without a continuous human expert supervision. Previously, these systems should assimilate the experts knowledge in order to provide an effective assistance and supervision. \sidenoteDavid{Nuevo}

%%%%%%%%%%%%%%%%%
% Version antigua
%%%%%%%%%%%%%%%%%
% \textcolor{blue}{Despite humans are still indispensable to develop complex tasks whose automation is not feasible yet, supervision systems have arisen as a suitable alternative to automatically assist humans when they are performing those tasks.} \sidenoteDavid{Lo he reescrito, ¿mejor así?}\sidenoteMj{rehacer la frase siguiente}In contexts where an appropriate use of abstract knowledge or an interaction capability with the surrounding environment are required by an operator or apprentice, those systems may be able to supervise whether a human is performing the task correctly, detect deviations from the established plan, and advice him or her in real time if that were the case. The training of new skills and the human errors during their execution could entail a high cost that could be reduced by automated supervision systems indicating when, where and how a protocol error takes place, in a comprehensible way for the user or the professional. \textcolor{blue}{This technology is specially applicable to supervise jobs under a well-defined workflow or strict protocol, or also for training environments where a continuous monitoring and feedback is the basis for a correct learning of procedures.}\sidenoteDavid{He usado esta frase del Explora. Creo que explica mejor la motivación de la supervisión automática} \sidenoteMj{rehacer la frase siguiente}Namely, it could be seen as an automatic expert in the matter made to help in this task and ultimately to enhance itself by supervision and guidance. These systems has been strengthen (mainly) by advances in the Activity Recognition (AR) field \cite{sukthankar2014plan}, which have provided with a wide range of approaches to recognise human activities in multiple domains, such as industry (\cite{marinho2017preliminary}, \cite{maekawa2016toward}%, \cite{roitberg2015multimodal}, \cite{wu2012automated}, \cite{petrovic2010context}
% ),  surveillance (\cite{batchuluun2017fuzzy}, \cite{kardas2017svas}, \cite{mabrouk2017abnormal}%, \cite{hu2013incremental}, \cite{zin2010markov}, \cite{ran2010applications}
% ), smart environments and daily-living assistance (\cite{chernbumroong2013elderly}, \cite{banos2012daily}, \cite{hoey2010automated}%\cite{ayase2008method}, \cite{camacho2014ontology}, \cite{brdiczka2009learning},  \cite{yordanova2017s}
% ), or medicine and health-care (\cite{sanchez2008activity}, \cite{corchado2010using}, \cite{negin2018praxis}%, \cite{nakawala2017development}, \cite{soutschek_measurement_2010}, \cite{hein_saphire_nodate}, \cite{dosis2005synchronized}, \cite{ghali2003object}, \cite{yordanova2017situation}
% ). The socioeconomic impact derived from automatic supervision %the latter 
% would be remarkable for many human daily situations, allowing the instant detection of a human mistake at work that can cause a risky situation, or assisting people during their task accomplishment by providing meaningful and comprehensible feedback. 

% Automatic supervisors usually work in two sequential phases. Firstly, the systems must learn the essence of how one task should be done (i.e., a model of the task), coded by a programmer or learnt from examples and procedures provided by experts. Secondly, once the different ways of performing a task have been learnt, the system should be able to supervise the task when it is performed by a user. As the user operates, the system will compare the ongoing actions with the generalised model and will spot the discrepancies and possible amendments in real time. Considering that there may be different ways of correcting a possible wrong action, the system must be able to generalise in such a way that goes beyond particular cases and `understand' the intermediate goals of a task.\sidenoteJose{Rewritten}
%learn all of them (\sidenoteMj{lo del parentesis lo he añadido yo}or at least the most extensively used)\sidenoteDavid{Ok} to perform a proper supervision.

% The extraction of a computational task model, in a way that allows a system to conduct supervision, is a topic widely addressed in the area of Activity Recognition (AR). Applications of AR have been proposed 
% for a wide range of domains, such as industry (\cite{marinho2017preliminary}, \cite{maekawa2016toward}%, \cite{roitberg2015multimodal}, \cite{wu2012automated}, \cite{petrovic2010context}
% ),  surveillance (\cite{batchuluun2017fuzzy}, \cite{kardas2017svas}, \cite{mabrouk2017abnormal}%, \cite{hu2013incremental}, \cite{zin2010markov}, \cite{ran2010applications}
%  ), smart environments and daily-living assistance (\cite{chernbumroong2013elderly}, \cite{banos2012daily}, \cite{hoey2010automated}%\cite{ayase2008method},  \cite{brdiczka2009learning},  \cite{yordanova2017s}, \cite{camacho2014ontology}
%  ), or medicine and health-care (\cite{sanchez2008activity}, \cite{corchado2010using}, \cite{negin2018praxis}). All these applications have been motivated (mainly) by the objective of allowing computing systems to  assist humans with their tasks. 
%  \sidenoteDavid{Nuevo}\sidenoteJose{Es Activity Recognition lo mismo que Automatic Supervision? Este párrafo da a entender que sí, y tira por tierra toda la novedad que podría tener el artículo en cuanto a supervisión, y los primeros párrafos. Para mí, activity recognition es parecido pero no lo mismo. Igual estoy equivocado, pero los nombres, al menos, son muy diferentes.}
 
 %, \cite{nakawala2017development}, \cite{soutschek_measurement_2010}, \cite{hein_saphire_nodate}, \cite{dosis2005synchronized}, \cite{ghali2003object}, \cite{yordanova2017situation}
%

% \sidenoteMj{Hasta el final de este párrafo hay que revisarlo}\sidenoteDavid{La he retocado, no sé si está más clara ahora.}\textcolor{blue}{In this way, the system should be capable not only of recognising the current state of the task, but also potential user's actions and goals. In short, the possible plans that lead the user to complete the task. In this context, Plan Recognition (PR) \cite{sukthankar2014plan} plays a fundamental role in the learning phase (the first one mentioned before) in order to generalise the execution of a given task.}


%%%%%%%%%%%% Version anterior %%%%%%%%%%%%

% These automatic supervisors usually work in two sequential phases. Firstly, the systems must learn the essence of how one task should be done (i.e. a pattern) from the examples provided by experts. Secondly, once the different ways of performing a task have been learnt, the system should be able to supervise the task executed by an apprentice by comparing her execution with the patterns learnt in the first phase. Therefore, considering that there may be different ways of correctly executing one task, the system must be able to learn all of them (\sidenoteMj{lo del parentesis lo he añadido yo}or at least the most extensively used)\sidenoteDavid{Ok} to perform a proper supervision. 
% %Therefore, considering that there may be different ways of correctly executing one task, the system must learn all of them to perform a proper supervision.
% \sidenoteMj{Hasta el final de este párrafo hay que revisarlo}\sidenoteDavid{La he retocado, no sé si está más clara ahora.}\textcolor{blue}{In this way, the system should be capable not only of recognising the current state of the task, but also potential user's actions and goals. In short, the possible plans that lead the user to complete the task. In this context, Plan Recognition (PR) \cite{sukthankar2014plan} plays a fundamental role in the learning phase (the first one mentioned before) in order to generalise the execution of a given task.}
%%%%%%%%%%%%


% ref para el párrafo\cite{chen2012sensor}

% \sidenoteJose{La intro no debería pasar de dos páginas y por fin parece que llegamos a la motivación del paper.}\sidenoteJose{Y párrafos de casi una página. Son infumables. Hay que ir al grano, sintetizar y trocear}
% According to the mechanism that is used during the learning phase, the AR approaches can be distinguished in data-based approaches and knowledge-based approaches \cite{chen2012sensor}. Traditionally, the AR applications have been dominated by the first one. These rely on an intensive use of preexistent data of users’ behaviours to obtain the task model. Data mining and machine learning techniques are used to create probabilistic or statistical models. % that are trained in a subsequent step. 
% Although both techniques are undoubtedly contrasted\sidenoteJose{lo de contrasted no creo que funcione en inglés. En cualquier caso, si funcionan no se motiva la segunda parte de la frase. ¿Tienen limitaciones, sí o no?}, the automatic supervision must go away from these methods\sidenoteJose{go away? rewrite...} if the supervision is expected to be general, transversal and pervasive enough to be tuned to multiple domains. This is motivated by several reasons. Firstly, many domains that could potentially  be benefitted by automated supervisors, are characterised by very little or sparse activity data. Although there are plenty of datasets about human activities \cite{chaquet2013survey}, this data becomes useless when the set of activities required to learn a task is specific to certain domain\sidenoteJose{No entiendo esta frase, me parece un poco contradictoria}. As a result, new data must be recorded and annotated. This process is costly and time consuming. Hence, supervision systems must learn from fewer supervised reference procedures to generalise the task. Secondly, the information necessary to make automatic supervision effective enough is not only in the observations. Tasks are more than a simple sequence of low-level actions. Indeed, they become intelligible to humans when certain level of abstraction is reached. The system should allow the definition of %deep concepts and 
% abstract knowledge in order to capture the intention and meaning of the user's actions. %ongoing performance of the user. 
% Moreover, assertive supervisors must go a step further than simple user's action recognition.\sidenoteJose{Aha... primera diferencia entre supervisor y recogniser... Pero llega muy tarde y de refilón} Deviation detection and proper feedback providing must be overhauled.\sidenoteJose{Frase no gramatical} Therefore, learning process\sidenoteJose{Learning o supervision? De todas maneras este desiderata suena a carta a los reyes} must become more cognitive and predictable, by taking more advantages of intentions, constraints, source and context of the data, rather than just looking at information as raw data. Finally, when only few observations are available, it becomes even more important to take advantage of the rich knowledge that domain experts can provide to the virtual supervisor.\sidenoteJose{Esto no se ha dicho ya? Este párrafo no acaba nunca} Appropriate learning mechanisms to acquire, codify and make use of the experts knowledge will be basis to that end.\sidenoteJose{Frase vacía} Alternatively to a data-driven approach, a knowledge-based approach makes use of those mechanisms to capture the prior knowledge in the domain to generalise the procedure to supervise.\sidenoteJose{De nuevo, esto no se ha dicho ya?} In those application domains, where automatic supervision must learn from a few reference procedures, the appropriate technology must be chosen to learn a model from incomplete information.\sidenoteJose{Frase vacía.} For that reason, an inductive approach\sidenoteJose{Qué es un "inductive approach", para mí es sinónimo de "learnign"} would be more suitable in order to fill those gaps by making the most of experts' experience and background. \sidenoteJose{En resumen, si queremos decir que nuestra propuesta recoge lo mejor de los dos mundos y consigue abstraer porque usa X, Y y Z, en vez de W, R y S no ha quedado nada claro.}
% \sidenoteDavid{Nuevo}

%%%%%%%%%%%%%%%%%
% Version antigua
%%%%%%%%%%%%%%%%%
% In those context in which the supervision system must learn from one correct reference procedure (or at most a few), automatic supervision must go away from classical machine learning and statistical modelling and use some other methods that allow the introduction of strong bias that is represented by the prior knowledge about the domain and environment.
% Though, nowadays, there are datasets with many human activities in different situations and scenarios to generate those model \cite{chaquet2013survey}, certain domain activities are so specialised that new data must be recorded and annotated. This is costly and timeconsuming. Additionally, it is a fact that people can perform certain activities significantly differently from others. Training data might not contain enough variants of the users plans to create a general model capable of expressing as many ways of performing the task as possible. This usually leads to models that are not scalable or reusable. Finally, supervising a task involves much more than a sequence of linked activities that can be derived from the data. Low-level actions makes it difficult to capture the intention and meaning of the ongoing performance of the user. 
% textcolor{red}{and a short-sighted reasoning  \sidenoteMj{la palabra reasoning tiene que explicarse. Te refieres a que los patrones no tienen en cuenta las acciones ni la tarea?} in regard to the actor's actions and the ongoing task. On one hand, most recognition algorithms require extensive amounts of training data. \sidenoteMj{las 2 frases que vienen a continuacion no se entienden}
% Although there are multiple datasets based on human activities for different situations and scenarios \cite{chaquet2013survey}, when certain tasks to be monitored entail a set of very specific activities, make the previous dataset useless to train a model for that purpose. Therefore, new data must be gathered and annotated, with the subsequent economic and time-consuming effort which it implies. Additionally, as in some human routines some people can perform certain activities significantly differently from others, training data might not contain enough variants of the users plans to create a general model that captures as many ways of performing the task as possible. \sidenoteMj{revisar hasta el final del párrafo}On the other hand, reasoning without enough abstraction (i.e., low-level reasoning) about user’s actions is not suitable to that end for several reasons. First of all, those systems tend to be more prone to noise from observation layer such as sensor data, video signal, etc. Second, they are usually designed for an specific domain application, discarding the generalisation mechanisms to ease the reusability of the acquired knowledge for other purpose. Moreover, complex activities are only recognisable at certain level of abstraction, thus a high-level reasoning in this regard enhance the capability of the system to offer valuable assistance when a skill-demanding task is being carried out by the user \cite{chen2012sensor}.} %Thus, it becomes necessary an abstract reasoning throughout the user task for providing a reliable supervision and assistance. 
%%%%%%%%%%%%%%

%\sidenoteMj{revisar esta primera frase}

% In this way, the system should be capable not only of recognising the current state of the task, but also potential user's actions and goals. In short, the possible plans that lead the user to complete the task. 

% It is a fact that for an effective supervision, it is needed to know all the different ways that lead the task to success and, in many cases, 

% \sidenoteJose{Zasca, qué cambio. Aquí se introduce para motivar o para explicar. Si es para explicar, deberíamos empezar con una pregunta, ¿cómo podemos integrar lo mejor de la aproximación basada en conocimiento y la basada en datos? Y aquí supongo que entraría inductive programming.}
% Inductive Programming (IP) \cite{gulwani2015inductive} is a research area where artificial intelligence, machine learning and cognitive science join in order to learn (small) %declarative
% programs from a small set of  examples and some declarative background knowledge. IP provides interesting features that can be highly exploited by the automatic supervision in order to acquire the expert's knowledge. Those systems can be supplied with a start-up knowledge (domain information) and then enriched incrementally by the system through the examples. In this manner, an expert could initially introduce the abstract knowledge, detailing the high-level concepts and task constraints, and then increment it (automatically) by recording some illustrative executions of how this task should be performed. Recently, \cite{monserrat2016knowledge} presented an IP approach that is able to learn automatically the relationships between some high-level activities (defined by the expert) and the observable events detected in video-recorded executions\sidenoteJose{O sea, no hay ya novedad y el problema está resuelto? Habrá que comentar sus limitaciones, no?}. In general, IP approaches rely on declarative languages (i.e., expressed as potentially comprehensible rules) to represent the examples, background knowledge and generalised hypotheses. Thus, the inferred programs can be inspectable and understandable by the domain experts. This would allow experts to monitor these rules and modify those that are not considered appropriate or do not fit the task. Also, declarative languages ease the use of inference mechanisms for logical reasoning (e.g., deduction, induction or abduction). These could be useful for making predictions about the user's behaviour or explaining the system decisions. \sidenoteDavid{¿Pongo alguna propiedad más?¿Cuál?}\sidenoteJose{No, creo que hay de más. Se está alargando mucho. La intro debe tener, problema, idea novedosa y cuatro pinceladas de la solución. Y ya está. Nos falta la idea novedosa, y tenemos trozos de la solución.}\sidenoteDavid{Nuevo}

% \sidenoteJose{Si este párrafo es el que tiene que explicar qué es realmente lo nuevo de este paper, a mí me parece todo generalidades... No va al grano ni del problema ni de la solución.}
% In spite of the possibilities of the IP automated supervisors, there is still a need for approaches that help those systems to bridge the gap between the observed executions from experts, and the logical knowledge acquisition. It is a reality that many contexts of supervision usually have just one correct reference procedure (or at most a few) to compare with, as this requires time and effort from experts. Additionally, some experts can perform the task significantly differently from others, being different plans possible on task accomplishment. Therefore, some kind of generalisation approach will be required to abstract the task structure (i.e., a pattern) from very few demonstrations, and consolidate it in the IP supervisor knowledge base. That means to develop the right mechanisms to put in common the different task observations, mining the dominant pattens, and filter the main steps from the superfluous ones. A refinement mechanism will also be necessary to search, in the space of possible solutions, the most accurate model according to the observed examples. Even when the discrepancies between plans are little or notably.\sidenoteDavid{Nuevo}



%%%%%%%%%%%%%%%%%%% Version MJ %%%%%%%%%%%%%%%
% Inductive Programming (IP) \cite{gulwani2015inductive} is a research area where artificial intelligence, machine learning and cognitive science join together in order to learn (small) declarative programs from a few observations and some declarative background knowledge. IP systems have been also shown successful for the automation of repetitive task in other human-related application domains, such as the FlashFill \cite{gulwani2011automating} and  FlashExtract \cite{gulwani2017framework} tools for data transformation, or the creation of educational content for different subjects (logic, programming or algebra) directly from examples \cite{gulwani2014example}. Needless to say, learning a complex task from a few instances in a physical environment entails many more challenges. However, we believe that this is possible if the training examples are sufficient meaningful for describing the task, an appropriate level of abstraction \sidenoteMj{reasoning?? No entiendo lo siguiente} is achieved, and the right tools and mechanisms are developed to acquire the knowledge of the experts in the matter \cite{monserrat2016knowledge}. But there is also still to bridge the gap between the observed information and the logical knowledge acquisition. Therefore, some kind of generalisation approach is required to that end; that is, put in common the different task observations, mining the dominant plans, and filter the main steps from the superfluous ones. In this regard, a refinement mechanism will also be necessary to search, in the space of possible solutions, the most accurate model according to the observed examples, even when they present little discrepancies between them, or notably different plans of performing the task.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%This challenge has characterised at length the research area of Inductive Programming (IP) \cite{gulwani2015inductive}, area where artificial intelligence, machine learning and cognitive science join together in order to learn human routines, in the form of computer programs, from several examples observations and some declarative background knowledge. IP is concerned about making expert systems learn programs automatically in situations where data become scarce. Moreover, experts knowledge can enhance significantly the system performance by introducing the domain constraints, as long as that knowledge is captured appropriately by the system. Inductive programming has been successful for repetitive task automation in other human-related application domains, such as data transformation tasks with FlashFill \cite{gulwani2011automating} or  FlashExtract \cite{gulwani2017framework} tools, or creating educational content for different subjects as logic, programming or algebra, directly from examples \cite{gulwani2014example}. Needless to say, learning a complex task from a few instances in a physical environment entails many more challenges, however, we believe this is possible if those examples are meaningful enough describing the task, an appropriate level of abstract reasoning is achieved, and the right tools and mechanisms are developed to acquired the knowledge of the experts in the matter \cite{monserrat2016knowledge}. But there is also still to bridge the gap between the observed information and the logical knowledge acquisition. Therefore, some kind of generalisation approach is required to that end; that is, put in common the different task observations, mining the dominant plans, and filter the main steps from the superfluous ones. In this regard, a refinement mechanism will also be necessary to search, in the space of possible solutions, the most accurate model according to the observed examples, even when they present little discrepancies between them, or notably different plans of performing the task.
% \sidenoteDavid{Corregido. Era un trozo de texto que se me había quedado sin comentar.}\sidenoteMj{No creo que haga falta mencionar ILP, aunque falta conexion con IP. Revisar rl resto de parrafo}\sidenoteJose{No, en la intro no más, por favor :-)}


% by developing inductive refinement techniques to find the most accurate model according to the observed examples in a search space of possible manners candidates. As in Inductive Logic Programming (ILP) 

% Mechanisms to But as in other inductive learning context, a general pattern is underlying the examples and must be present in each relevant observation  inductive refinement techniques to find the an underlying representation and most accurate according to the observed examples.

% , all this in order to synthesise the task in a general representation. In  a first incursion in inductive supervision were achieved, where obtained from some meaningful examples performed by skilled experts on the matter, which lend it to be considered as the correct way that must be followed to perform the task under supervision in the proper way . Nevertheless, 
% Nevertheless, mechanism to deal with  and the search space of possible manners of developing it are sufficiently delimited for the system. In this sense, %Inductive Logic Programming (ILP) \cite{muggleton1994inductive} provides 
% some inductive refinement techniques to find the an underlying representation and most accurate according to the observed examples.

% Even though a task can be performed in different ways, we believe that a general pattern underlies them and must be present in each relevant observation. Therefore, there is still necessary to bridge the gap between the observed information to the logical knowledge acquisition with some kind of generalisation mechanism. In supervision contexts where data is lacking and the supervised task is skill demanding for humans, new methods are required to put in common different observations, mining the dominant ways, and filter the main steps from the superfluous ones.

% On the other hand, existing literature in PR (\cite{yang2007learning}, \cite{yang2005learning}, \cite{blythe2001integrated}, \cite{benson1995inductive}, \cite{wang1995learning}) have shown it is possible to acquire the missing knowledge concerning tasks by learning from plan observations. 
 % Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.   %Therefore, there is the possibility of capturing that essence from several but ``rich'' examples. Nonetheless, in supervision contexts where data is lacking and supervised task is skill demanding for humans, there still necessary to bridge the gap between the observed information to the logical knowledge acquisition with some kind of generalisation mechanism. New methods are therefore required to put in common different observations, mining the dominant ways, and filter the main steps from the superfluous ones. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.   

% \textcolor{blue}{David: Voy a reescribir esta parte. Creo que quedará mejor juntandolo con el párrafo anterior}\\
% In order to address this generalisation challenge, the contribution of this paper is twofold: (1) we present a novel inductive approach\sidenoteJose{No sé lo que es un "inductive approach". Es un machine learning approach? o es un "inductive programming approach"? } to extract the underlying  \FullNamePlanSpaceGraph{s} \textcolor{blue}{[quizá denominarlos como (\ShortNamePlanSpaceGraph) o Plan Space Models (PSM)]}\sidenoteJose{Esto ni se ha motivado ni conectado con nada de lo anterior. Llevamos tres páginas y cuando llegamos a las contribuciones, no sabemos que es un PSM... ni por qué hacen falta. El título va de plan patterns... y no se ha explicado qué es. Y estamos en la página 4!} from a set of labelled human activity sequences until all the examples are covered by at least one of those patterns. As an outcome, we get multiple ``compact'' \footnote{we use this term in this paper to mean a smaller size compared to the addition of individuals}\sidenoteDavid{¿Entonces dónde indico esto? Me parece interesante aclarar este concepto.}\sidenoteMj{la footnote no se entiende y ya antes se ha mencionado compacteness} plan patterns, where the main activities and their relationships are kept on it. This allows us to filter the superfluous information that is not strictly necessary to learn the task; (2) we study the coverage of those models according to new instances unseen by those patterns. For this purpose, we use several state-of-the-art metrics from graph theory domain to measure the similarities between a \ShortNamePlanSpaceGraph{} and a given plan %graph 
% instance. All this will be enable us to take a further step towards a real automation of the learning phase\sidenoteJose{automation of the learning phase? Eran los otros métodos manuales?} along the supervision process. Furthermore, our approach makes it possible to deal with the lack of examples and the divergence of ways to perform a skill-demanding\sidenoteJose{skill-demanding?} task. The potentiality of this method will be tested in one domain characterised by the prior handicaps\sidenoteJose{prior handicaps? No entiendo.}: the automatic skill supervision in surgical training tasks. 

% •	Recognise sequences of gestures that are new to the system.
% •	Recognise repetitions.
% •	Detect boundaries of a task.
% •	Identify the optimal representation for a certain task.

% How to get the general planning of a task through a few example sequences?
% How to avoid/reduce the noisy transition between actions of the sequences?


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Párrafo para 
% In literature exists a considerable number of approaches for modelling human plans. 

%Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.  

% in the transition from the detected information to the logical knowledge acquisition in AR is still necessary to design mechanisms, not only to provide the task boundaries, but also to identify an optimal representation of them. Therefore, generalisation methods are required to join the different executions, mining the dominant ways, and filter the main steps from the superfluous ones. This would provide a good initial guess about which activities, together with their relationships, compound the route map where the task steps must flow to fulfil it. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.  Then, given the fact the task is known, the following step is to identify and learn the patterns of correct ways (i.e., the form of the plans) that could achieve the task goal. Nevertheless, the huge challenge here is addressing this objective in contexts where data is lacking. the task is skill demanding and there are multiple forms to perform it. New methods are required to join the different executions, mining the dominant ways, and filter the main steps from the superfluous ones. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.  

% In this way, graph analysis provides multiple features to extract meaningful information from connected structures such a sequence of steps does. Thus, some noteworthy fields such as bioinformatics [ref], social-network analysis [ref], computer vision [ref] and image processing [ref] have taken advantage of these capabilities. Subgraph finding, for instance, enables us to discover recurrent patterns that are hidden in a set of graphs [ref]. In turn, graph comparison is used to group similar graphs into clusters applying a similarity criterion [ref]. Despite the fact that these features are powerful, they are computationally expensive, as the size of the graph grows (NP-hard). Many researches during last decade have provided a wide range of kernels to address this problem.
   
%\textcolor{red}{FALTARÍA ESPECIFICAR EN QUÉ PARTE SE VA A CENTRAR EL ARTÍCULO. Nos vamos a centrar en la parte de aprendizaje y, en concreto, la parte de "aprender" todas las formas de realizar una tarea de forma correcta a partir de unos pocos ejemplos introducidos por los expertos. Además, habría que resaltar que el método de aprendizaje no estaría limitado a la fase de entrenamiento sino que se podría seguir durante toda la vida útil del sistema mientras le sigan llegando ejecucciones correctas llevadas a cabo por el sistema. Además, el aprender todas las formas de realizar correctamente una tarea también es algo que diferencia nuestro sistema de uno de automatización de tareas. En la automatización basta con aprender como ejecutar una tarea correctamente. Además, precisa de aprender todos los detalles de esa tarea. En Supervisión, hay que aprender todas las formas de llevar a cabo una tarea pero no hace falta aprender el detalle, basta con aprender los pasos clave para conseguir llevar a cabo la tarea con éxito. El aprender todas las formas de realizar la tarea y diferenciar entre los pasos clave y los superfluos son los objetivos del trabajo que se presenta en este paper.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Motivation} \label{motivation}

Learning the process that underlies a human task from the observation of a few correct executions is a complicated challenge for a machine. Something that humans can do naturally and easily, such as identifying what is required to complete a task (i.e, actions, objects, intermediate states) with just a couple of examples, for a machine is a real challenge of abstraction and generalisation. Although the steps of the task can be specified and clear, two execution examples can perform sequences of very different activities that meet the specifications. These differences are usually motivated by the small differences in the initial stages in each example, the degree of freedom offered by the task, the previous experience of the person executing it or the interpretation that this makes of the instructions. In this process of generalisation, a human solves in a natural way the points in common and the differences between the observations, creating an abstract scheme of what he needs to be able to perform the task and the ways he could do it. 

How to perform this generalisation in order to make a system learn the task is not trivial for some context. Specifically, if this system has to make decisions to assist people. Let us imagine a scenario where a system has to supervise if a person is cooking right a carrot soup. Table \ref{tbl:cooking_vocabulary} shows the vocabulary of activities that are involved in this task. Previously, the system has observed the following two examples of how to cook this dish (in the form of sequences of activities): ``$SABCDFGHIMOPT$'' and ``$SABCEFGJKLNOPT$''. These examples show two forms of cooking: using a microwave or using the kitchen stove. One could think of a possible generalisation is ``$SABC \{D|E\}FG\{HIM|JKLN\}OPT$'', where ``|'' means a disjunction between two activity groups for that portion of the task. As can be seen, this generalisation considers both examples as valid, but it also covers other cases that are far for being safe for the person who is cooking. For instance, the sequence ``$SABCEFGHIMOPT$'', where the person takes a metal pot to put inside the ingredients and then put the metal pot into the microwave to prepare the soup. The system would give it as a valid sequence following the model above, but these actions are completely contraindicated for the task that is intended. 

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{table}[!t]
\centering
\resizebox{12cm}{!}{%
\begin{tabular}{cl}
\multicolumn{1}{l}{Activity Code} & Activity Description \\ \hline
S & Start the task \\
A & Peel the carrot \\
B & Wash the carrot \\
C & Cut the carrot into pieces \\
D & Take a glass pot \\
E & Take a metal pot \\
F & Fill the pot with water \\
G & Add salt \\
H & Put the pot into the microwave. \\
I & Turn on the microwave to the maximum (15 minutes). \\
J & Put the pot on the stove \\
K & Turn on the stove to the maximum (10 minutes). \\
L & Reduce the stove to the minimum (30 minutes). \\
M & Turn off the microwave. \\
N & Turn off the stove. \\
O & Take a deep dish. \\
P & Add two large spoonful of soups on the dish. \\
T & Finish the task
\end{tabular}%
}
\caption{Vocabulary of activities for cooking a carrot soup. }
\label{tbl:cooking_vocabulary}
\end{table}

Thus, because the lack of negative examples, the solution must be as accurate as possible (being as close as possible to the observed examples), while ensuring the generality that is intended for supervision (determine those key steps for the task and how they are reached by following the previous ones). Therefore, every "generalisation" that is found must be supported by at least one positive execution in order to demonstrate that this generalisation really shows a plausible way to accomplish the task. In addition, there is the possibility of the presence of "non-essential" activities that should be suppressed during the learning/generalisation process of the task.

In summary: the need to learn from few examples, all positive, learning the different ways of executing a task and the possibility of the presence of noise (in the form of non-essential activities) at the same time is a complex task that does not solve the tools currently existing. That is why the need for the developments described in this paper has arisen.


==> sections/introduction_new.tex <==
\section{Introduction} 
\sidenoteCesar{he eliminado muchas referencias, en la intro para un concepto, con una referencia es suficiente}
%During the last decades, humans have tried to make possible the idea that a computer would be able to automatically perform tasks and activities that help humans in their daily lives. Nowadays, there are multiple fields of research devoted to the conception and developing  of automatic systems that monitor, recognise and respond to human behaviour, such as {\em Ambient Intelligence} \citep{camacho2014ontology} and {\em Context-aware systems} \citep{hong2009context}, {\em Advanced Driving Assistants} \citep{vskrjanc2018evolving} or {\em Surveillance systems} \citep{kardas2017svas}. Artificial Intelligence (AI), and more precisely Machine Learning,  provides the technology for conceiving intelligent agents able to recognise not only human actions, but also to understand their meaning and implications. 
In the past few decades, there have been important advances in making intelligent systems capable of automatically assisting humans in their tasks\sidenoteJose{Muy bien, pero por qué es importante este problema?}. These systems make use of Artificial Intelligence (AI), and more specifically Machine Learning, to recognise the actions humans make but also their meaning and implications. Research in this direction can be found in many research fields such as {\em Ambient Intelligence} \citep{camacho2014ontology}, {\em Context-aware systems} \citep{hong2009context}, {\em Advanced Driving Assistants} \citep{vskrjanc2018evolving} or {\em Surveillance systems} \citep{kardas2017svas}, to name a few. Before\sidenoteJose{Before? Como se puede aprender nada antes de monitorizar? No entiendo.} monitoring the human behaviour, the system must learn which activities are necessary to accomplish the task and their sequentiality
%what order relationships exist between them 
(that is, the \textit{activity workflow} of the task). Since a task may be performed in multiple ways, the agent\sidenoteJose{Quien es el "agent"? Te debes referir al automated assistant, creo yo} must be aware of the possible workflows that represent these ways.  \sidenoteDavid{He añadido este remate para acotar el tema a la fase de aprendizaje y no tanto al reconcoimiento.}

%\citep{mabrouk2018abnormal}. 

%Artificial Intelligence (AI), and more precisely machine learning,  provides the technology for conceiving AI agents able to detect and recognise not only human actions, but also to understand their meaning and implications. Traditionally, the area of Activity Recognition (AR) \citep{sukthankar2014plan} has addressed this kind of learning problems. Two approaches have been proposed:  data-based approaches, that apply well-known machine learning techniques for generating task models\sidenoteDavid{Traer refs del background},  and knowledge-based approaches \citep{chen2012sensor} that can use previous knowledge (bias) about the domain as a resource to generalise or learn the task\sidenoteDavid{Traer refs del background}. A somehow similar learning problem that applies machine learning techniques \sidenoteMJ{completar y mejorar con literatura} is Process Mining \citep{van2016process}. This emerging research area aims to discover, monitor and improve real process models (i.e., BPMN, EPC, UML, Petri nets, etc.) from event logs of systems\sidenoteDavid{}, and that has been successfully applied mainly in the area of business management \citep{van2007business} and health-care \citep{mans2008application}. \sidenoteMJ{David: añade referencias bibliograficas} \sidenoteDavid{Añadidas referencias y completado.}

%\sidenoteDavid{He reescrito el párrafo siguiendo la idea de Cèsar de solo una referencia, pero reperando la idea original de comentar los dos tipos de approaches.}

Traditionally, the area of Activity Recognition (AR) \sidenoteJose{Si "AR" sólo se usa unas pocas veces es mejor no usar siglas}
\citep{sukthankar2014plan}\sidenoteJose{Ahora se introduce esta área, cuando en el párrafo anterior se ha introducido otras áreas. Es esta la mejor? Es esta la que integra el problema? O es esta de la quese debe nutrir las anteriores, porque el primer paso es reconocer las actividades?} has addressed the problem of learning complex human task in order to recognise them\sidenoteJose{Se aprenden para reconocerlas? Es una "task" lo mismo que una "activity" o "task" es un conjunto de "activities"... Arriba se ha usado el termino task para todo (por ejemplo "activity workflow of the task", y aquí parece que es al revés. Aprovechemos para definir las cosas bien, p.ej., la wikipedia es muy clara: "aims to recognize the actions and goals of one or more agents from a series of observations on the agents' actions and the environmental conditions.". No hace falta eso, pero la primera frase podría ser: "A fundamental subproblem that appears in all the areas and applications above is known as Activity Recognition \cite{..}, which consists in the identification of a sequence of atomic activities (e.g., open a door) from observations coming from sensor logs, videos or other sources."}. %the recognition of complex human activities. % through two types of approaches: 
In AR, a distinction is made between data-driven approaches and knowledge-driven approaches. Data-driven approaches  (e.g., \citep{hoey2010automated}) are characterised by using supervised  machine learning techniques (mostly based on Markov models) for learning activity models from datasets of users’ behaviours.
%using supervised techniques based mostly on Markov models.
 These models provide high\sidenoteJose{high? Queremos decir good?} recognition results when facing uncertainty and temporal information but they require large-scale datasets to achieve a positive performance. In addition, such models are difficult to be applied from one person to another since they do not facilitate the incorporation of prior domain or expert knowledge\sidenoteJose{No entiendo esta frase... Difíciles de transferir? Pero la culpa la tiene el domain knowledge? Entre dos personas diferentes? Por qué? Si esta aproximación se realiza sobre muchísimos ejemplos, de entrada no podrían ser de una persona solo. No tiene sentido.}. %This dependency of data makes data-driven approaches to be sensitive to issues such as data scarcity or even the ``cold start''\footnote{This problem emerges when a data-driven application does not have the minimum amount of data to learn the task and operate. More information about this problem in \citep{chen2012sensor}.}\sidenoteDavid{He pasado esta definición a footnote para ahorrar un poco de espacio.}\sidenoteCesar{ esta frase la quitaría, ya sabemos que necesitan datos}\sidenoteDavid{¿Te refieres a la footnote? Si te refieres a la frase que la contiene, se me comentó que debíamos de hacer énfasis de las limitaciones que tienen.}
%, which is very useful when the amount of training data is small. However, %% siempre es útil, no?
\textcolor{blue}{In contrast, knowledge-based approaches (e.g., \citep{chen2008logical}) are characterized by exploting domain knowledge by using ontologies or logic formalisms (e.g., Event Calculus, Lattice theory, etc.)\sidenoteJose{Lattice theory sirve para construir modelos? Y event calculus? Será para "representar" los modelos, o representar el conocimiento, no? De hecho ahora se dice en la siguiente frase} to build %activity 
models. %  that consist of rules that define tasks and constraints by using ontologies or logic formalisms (e.g., Event Calculus, Lattice theory, etc.). Thus,   
%Hence, The
Ontologies and logic programs are suitable mechanisms to incorporate the
 expert knowledge into the learning process when there is not much data available.   %when there is little data and a .% is available.
Nevertheless,  %and it can be coded. However, training with little data makes knowledge-based approaches sensitive to infrequent behaviours %outliers 
these approaches still require programmers\sidenoteJose{No tienen por qué ser programadores. No creo que una "lattice" sea un programa. Seria suficiente decir que capturar el conocimiento del dominio es costoso y punto.} to code the expert's knowledge into the system.}\sidenoteDavid{revisar enfoque.}\sidenoteMJ{ya lo he revisado yo y lo he cambiado un poco}

%because they allow the use of domain knowledge in form of  activity models. The models  However, they are very sensitive to outliers in training data and they still require human programming of the system logic.

% Versión de Cèsar (solo con un % delante)
%===================================
%%Most of this systems should learn the way in that humans do the task in order to automatize it. Artificial intelligence and Machine Learning in particular provide with methods and techniques for learning task from a collection of examples that illustrate 
%%\sidenoteDavid{Dividir este parrafo en dos: AR y Process Mining. Orientar los párrafos sobre en qué métodos o técnicas se basan (e.g., tipos de técnicas como HMM).}
%%\textcolor{blue}{PÁRRAFO AR}\\
%Artificial Intelligence (AI), and more precisely Machine Learning,  provides the technology for conceiving intelligent agents able to recognise not only human actions, but also to understand their meaning and implications. Traditionally, the area of Activity Recognition (AR) \citep{sukthankar2014plan} has addressed this kind of learning problems. 
%%The current AR approaches can be grouped in data-driven approaches and knowledge-driven approaches \citep{chen2012sensor}. Data-driven approaches (\citep{hoey2010automated}, \citep{sanchez2008activity}, \citep{patterson2005fine}, \citep{kruger2014computational}) are characterised by using supervised (e.g., Hidden Markov Models (HMM), Linear Dynamical Systems (LDSs)) and unsupervised (e.g., KNN) machine learning techniques to address the problem. 
 %AR tools  provide high recognition results when facing uncertainty and temporal information but they require large datasets to achieve a positive performance. 
 %%This dependency of data makes data-driven approaches to be sensitive to issues such as data scarcity or even the ``cold start'' problem: the problem that emerges when a data-driven application does not have the minimum amount of data to learn the task and operate. In addition, such models do not facilitate the incorporation of expert knowledge, which is very useful when the amount of training data is small. 
 %However,
 %Knowledge-based  
 %%(\citep{okeyo2011ontology}, \citep{ye2015usmart}, \citep{chen2012knowledge}, \citep{chen2008logical}, \citep{bouchard2006smart})  
 %approaches \citep{chen2008logical}  are suitable when there is little data because they allow the use of domain knowledge in form of  activity models.
 %The models consist of rules that define tasks and constraints by using ontologies or logic formalisms (e.g., Event Calculus, Lattice theory, etc.). However, they are very sensitive to outliers in training data and they still require human programming of the system logic.
%%\sidenoteCesar{Metemos demasiadas referencias y explicaciones sobre otros trabajos, deberían ir al trabajo relacionado.}
%%\textcolor{blue}{PÁRRAFO SOBRE LEARNING BY EXAMPLES (IMITATION LEARNING + PM)}\\
%==================================

%%% NADA DE IMITATION LEARNING %%%%


%An alternative way to build an agent able to solve more or less complex tasks is by providing demonstrative examples of how humans perform such task. 
An alternative way to transfer the knowledge from experts to the system is by providing demonstrative examples of how humans perform the task\sidenoteJose{Aquí me muero... Esto es justamente lo que hace el "data-driven". Entonces para qué ha servido el párrafo anterior? Entonces esta es una manera alternativa al data-driven, al knowledge-driven, a los dos, o a qué?}. %to be supervised. 
%In this way, the human knowledge is transferred into the learning process through the examples used to train the models. 
This is the idea underlying %to the 
{\em Imitation learning} \citep{hussein2017imitation} and {\em Learning from demonstration} \citep{argall2009survey}, which are techniques that have been mainly applied for machines (robots in many cases)\sidenoteJose{Si no es para máquinas para qué es? No tiene sentido. Son máquinas siempre (no "mainly").} learning the necessary movements (i.e., policy)\sidenoteJose{Ya hemos hablado de workflow, process, task y ahora policy... O sea, un festival...} to solve a task. Many of these techniques are based on deep learning methods\sidenoteJose{Vamos, estas son "data-driven". Más claro el agua. Estamos dando círculos. Hay que reescribir estos dos párrafos--- Reducir si es posible. Se está haciendo muy largo, y abajo viene la motivación y el ejemplo, que es lo bueno}, which require large training data. Additionally, the comprehensibility of the induced models is poor which can be a handicap when trying to explain the system decisions.


%One way to automate the above is to learn from a few demonstrative examples provided by experts, or imitation learning \citep{hussein2017imitation}.
%Currently, this has been approached from the point of view of imitation learning \citep{hussein2017imitation}. \citep{xu2018neural} \citep{duan2017one} \citep{finn2017one}. 
%By using deep learning techniques, a machine (robots in many cases) can learn the necessary movements (i.e., policy) to solve a simple task through examples that show how to do it. These techniques, however, are limited 
%Although they have given surprising results even in scenarios with few examples, the tasks they are able to learn and 
%% to solve very basic tasks (e.g., stacking boxes). Many of them are based on deep neural networks, where the comprehensibility of the induced knowledge is poor. This factor is very important in cases where experts need to understand why the system makes certain decisions.
%\sidenoteDavid{He reescrito la frase que había.} to solve very basic tasks (e.g., stacking boxes) and the induced knowledge cannot be audited by humans. This auditory is very important in cases where experts need to understand why the system takes certain decisions and fix them if they have been wrongly learnt.

%%%%%% PÁRRAFO PROCESS MINING %%%%%%%%
%\sidenoteDavid{Cambiar como se introduce este párrafo}\sidenoteMJ{Ya lo he cambiado yo y he añadido el de imitation learning antes que al final me ha parecido que a algun revisor le puede faltar} A somehow similar learning problem %that applies machine learning techniques
%from demonstrative examples is Process Mining (PM) \citep{van2016process} which has been used to help organisations to reveal their business processes. The aim of PM is to discover, monitor and improve real process models ( %i.e., BPMN, EPC, UML,
%i.e. Petri nets) from traces of events (usually logs) that represent the sequence of activities that the expert has performed in a task demonstration. The techniques proposed in PM are based entirely on algorithms that allow traceability and analysis of the entire learning process, %process of generalisation,
%from the sequences to the final model obtained.  
%%%%%% %%%%%% %%%%%% %%%%%% %%%%%% %%%%%%


%In this approach the induced knowledge is easily interpretable by humans, being also easily processable to obtain other representations (e.g., logic rules). %The main difference with deep learning methods (black box models), is that the techniques proposed in process mining are based entirely on algorithms that allow traceability and analysis of the entire process of generalisation, from the sequences to the final model obtained. In turn, the proposed models are easily interpretable by humans, being also easily processable to obtain other representations (e.g., logic rules). \sidenoteDavid{He descomentado la mención a la esta parte }
\sidenoteCesar{Yo quitaría a partir de "the main difference", repite lo que hemos dicho ya, es redundante}
\sidenoteMJ{Quitado}

%However, in some contexts, the learning of tasks from execution examples performed by humans has some particular characteristics that make it different from other learning problems: (1) it is usually complicated or expensive to collect a large set of examples from experts in order to train the AI agent,  and (2) there is no unique way to perform a task but rather different experts could have different styles of making the task being all of them perfectly correct.  Thus, although data-based approaches have been the predominant way to generalise human tasks, they  require a large amount of pre-existent data from users’ activities, which makes them unsuitable to be applied for domains where there is not enough data.
%Analogously, logic-based approaches have problems in handling examples that represent different and/or infrequent user' habits of performing the activity. 

%However, in some contexts, the learning of tasks from execution examples performed by humans has some particular characteristics that make it different from other learning problems. 
 The previous approaches are not always able to deal with
characteristics commonly found when facing the learning of some real-world tasks from execution examples performed by humans.
\sidenoteDavid{No sé muy bien que se quiere decir con esta frase. Antes estaba la parte comentada de arriba.}
\sidenoteCesar{lo reescrito, pero es tampoco me acaba de convencer}\sidenoteMJ{He añadido lo de los ejemplos para que se entienda }\sidenoteJose{Yo no la entiendo, ya que hablamos de ejemplos, podríamos poner alguno? Yo en este punto de la intro ya me falta aire.}
First, in most contexts, even though the task is clearly specified, two experts can perform the same activity in a very different way, 
% that meet the specifications showing  that there are different styles of making the task, 
being both of them valid. Those differences may be due, for instance, to the degree of freedom of the task description, or diverse experiences of the experts\sidenoteJose{son los expertos? O son los operarios? Y realmente queremos decir "diverse experiences"? Eso se interpreta como experencias vitales. Igual lo que se quiere decir es "or different expertise levels"? Pero no estoy seguro de que sea eso."}. 
%or the interpretation that she makes of the task instructions. 
Second, it is usually complicated or expensive to collect a large set of examples from experts. And third,   collected examples are mostly or only positive, i.e., 
%show  sequences of actions or activities that allow to fulfil  tasks, but 
there are no examples that represent sequences of
wrong trials.\sidenoteJose{Reescrito}\sidenoteJose{Primer párrafo claro y motivador hasta ahora!}
%actions with which it is impossible to perform the task, 
%in other words, there are not negative examples. 

Let us illustrate the case with an example. 
%consider this example.
Imagine a scenario where a system has to supervise the task of cooking a carrot. Table \ref{tbl:cooking_vocabulary} shows the vocabulary of activities involved in this task. We have two examples of how to cook this dish (expressed as sequences of activities): ``$SABCDFGHIMOPT$'' and ``$SABCEFGJKLNOPT$''. These examples show two %diverse
different\sidenoteJose{dos maneras diversas no es lo mismo que dos maneras diferentes!}
forms of cooking: using a microwave or a kitchen stove, respectively. If we want to learn a general rule from these two examples, a possible generalisation %(process model or workflow) 
is the expression ``$SABC \{D|E\}FG\{HIM|JKLN\}OPT$'', where ``|'' means a disjunction between two activity groups for the portion of the task delimited by curly brackets. The two given examples are covered by the model, but there are  other  valid sequences of activities according to this model  that are not safe. For instance, the sequence ``$SABCEFGHIMOPT$'', where the person takes a metal pot,  put the ingredients in, and, then, put the metal pot into the microwave to prepare the soup. 
%, is covered by the above workflow although these actions are not recommended for cocking because its potential risk. 
We need a learning procedure and a representation language that is able to find the right trade-off between an overgeneralisation covering almost everyting and an overspecialisation that is simply the alternative between the two sequences.\sidenoteJose{He reescrito esto, pero estaría bien ver que también hay un riesgo de overspecialisation, por ejemplo “{SABCDFGHIMOPT|SABCEFGJKLNOPT}”, cuando lo que se quiere es algo como “SABC{DFGHIM|JKLN}OPT”, no? En cualquier caso sería interesante poner algún ejemplo con ruido, por ejemplo "BB" }  To avoid an overgeneralisation, given that we do not have negative examples, the model should be as close as possible to the observed examples.
%while ensuring that is enough general for not including unnecessary activities. 
But, at the same time, the generalisation should be able to capture the two ways of cooking a soup shown by the examples. % to also cover other unseen sequences of activities that properly perform this task.   %The system would consider it as a valid sequence according to the above model, but these actions are completely contraindicated for the task that is intended. 

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{table}[!t]
\centering
\resizebox{10cm}{!}{%
\begin{tabular}{cl}
\multicolumn{1}{l}{Activity Code} & Activity Description \\ \hline
S & Start the task \\
A & Peel the carrot \\
B & Wash the carrot \\
C & Cut the carrot into pieces \\
D & Take a glass pot \\
E & Take a metal pot \\
F & Fill the pot with water \\
G & Add salt \\
H & Put the pot into the microwave. \\
I & Turn on the microwave to the maximum (15 minutes). \\
J & Put the pot on the stove \\
K & Turn on the stove to the maximum (10 minutes). \\
L & Reduce the stove to the minimum (30 minutes). \\
M & Turn off the microwave. \\
N & Turn off the stove. \\
O & Take a deep dish. \\
P & Add two large spoonful of soups on the dish. \\
T & Finish the task
\end{tabular}%
}
\caption{Vocabulary of activities for cooking a carrot soup. }
\label{tbl:cooking_vocabulary}
\end{table}

\sidenoteJose{Las descripciones de las actividades de cocina son Spanglish, no? Me partía leyéndolas :-) "to the maximum" -> "at a maximum level"... "deep dish" -> "deep saucepan" o "deep bowl"?? Generalmente los dish son "shallow" :-) Suena raro. Y la mejor es:  "two large spoonful of soups" si es "dos cucharadas soperas" es simplemente "two tablespoons" :-)))) }

 %Consequently, learning the process that underlies a human task from the observation of a few correct executions is a complicated challenge for a machine. Although data-based approaches have been the predominant way to generalise human tasks, they  require a large amount of pre-existent data from users’ activities, which makes them unsuitable to be applied for domains where there is not enough data. Analogously, logic-based approaches and traditional process mining techniques  have problems in handling examples that represent different and/or infrequent user' habits of performing the activity.
 
 %As shown by the example, automatic supervision systems is an application domain in that all the above-mentioned characteristics hold.  The automatic supervision of monotonous and/or complex processes could be a reasonable alternative when the complete automation of a task is not feasible because it would require appropriate use of abstract knowledge, a capability of interaction with the surrounding environment, or the handling of uncertainty. Some applications of these systems can be found in health care  \citep{hoey2010automated}, \citep{bouchard2006smart}, \citep{su2014kinect} \citep{tang2015physio}, smart homes/environments \citep{twomey2016sphere}, \citep{intille2006using}, \citep{krose2008care}, \citep{crandall2011tracking} or cooking labours \cite{kruger2014computational}, \cite{yordanova2017s}, \cite{neumann2017kognichef}. Supervision systems, after the observation of how an expert performs a task, are able to supervise whether other humans are performing this task correctly, also by observation. Note that, for effective supervision, the system must be first able to learn all the different ways the task could be performed according to the expert observations.\sidenoteDavid{Movería este párrafo a las conclusiones y lo extendería con las posibilidades de nuestro sistema de supervisión.}\sidenoteMJ{David: en este párrafo se pueden añadir algunas referencias a sistemas de supervision ()}
 
 In this paper, we aim to define a mining approach\sidenoteJose{No me gusta la construccion "mining approach", qué es un "mining approach"... Minería tradicional? O es un "data mining approach"? , que no es lo que hacemos, o es un workflow mining? Y si es así, qué es workflow mining? No se ha explicado y está en el título.}  able to extract all the essential ways to perform a task from a few expert executions. The novel method overcomes many limitations of the existing
 %data-based,  knowledge-based, and existing process mining 
 approaches by defining a learning method based on inductive learning\sidenoteJose{Learning es siempre inductive, esto no tiene sentido...}, graph theory\sidenoteJose{Realmente usamos teoría de grafos?} and process mining %. Process mining is 
 (a research area focused on discovering %, monitoring and improving 
 a general %single 
 business process model %( i.e., BPMN, EPC, UML, Petri nets) 
 from traces of activities that show the behaviour of the system users).\sidenoteJose{Ahora por fin introducimos "process mining" (que no workflow mining) en un paréntesis y de refilón....}
 %(usually logs) 
 %with the behaviours of the business system users. 
 %Compared with process mining, the examples from which we start are intentional demonstrations of the task provided to the system in order to learn the possible workflows.
 \sidenoteDavid{He traido lo de process mining aquí.}\sidenoteMJ{he borrado una frase que me parecía redundante ya que al principio del parrafo ya decimos que los ejemplos son ejecuciones de los expertos}  As a result, we infer multiple %workflows or 
 models in the form of dependency graphs 
 %\citep{van2004workflow}, \citep{agrawal1998mining}, \citep{schumann2013distance},
 \citep {agrawal1998mining}, a typical representation for process models where the graph nodes represent the involved activities, and the directed arcs represent an order relation between these activities. This notation has two advantages:  graphs are easily understandable and make it possible to filter the non-essential activities \citep{van2016process}. One activity is considered non-essential if its execution is not necessary to finish the process correctly. 
 %The algorithm also ensures the validity of each extracted model as a complete representation of one specific way of carrying out the process, and its feasibility by checking that, at least, one training example is represented by at least one of the output models. Finally, we have analysed some properties of the resulting models: their  generalisation capability, their simplicity and their fitness to the training examples. 
 As far as we know this is the first approach that proposes the combination of dependency graphs and an inductive method\sidenoteJose{Creo que "inductive method" no dice nada, y hemos comentado "process mining for learning tasks". Learning es inductivo generalmente. Uno puede memorizar, pero eso no es learning en mi opinión, si no hay inducción. Mining is inductive siempre... Creo que hay un lío terminológico aquí monumental...} for %process modelling 
 learning tasks performed by humans. %in a knowledge-based supervision system.
 %To %analyse the applicability of the model, we have
 We show the potentiality of our method by applying it on a very challenging environment in that all the previously mentioned issues\sidenoteJose{Convendría recordarlas, se han nombrado dos párrafos antes. Si nos referimos a multiple ways of solving a task, positive examples only, and very few examples. En cualquier caso falta justificar mejor por qué dependency graphs es la solución para esto... Es una elección como cualquier otra. Y si no lo es, no está justificado.} are present: a surgical training task.
 
 \sidenoteJose{Título y abstract usan workflow mining, y aparece process también. Y hasta aquí ni se ha visto... Hay unos choques terminológicos brutales...}

The rest of this paper is organised as follows.  %in the following manner. Section \ref{motivation} presents briefly the motivation of this work. In this section we want to answer the question of why we have developed this research.
Section \ref{matandmet} presents  our Mining Multiple Workflows (MMW) approach based on dependency graphs.
%: we firstly introduce the graph-notation, some related definitions, and the data formalisation, and then we define the mining method. 
Section \ref{s:results} presents the experimental setup and the results of applying our approach with a set of real examples taken from laparoscopic surgery training. In Section \ref{s:discussion} we discuss the experimental results and the strengths and limitations of our method. %Section \ref{background} reviews the literature on activity recognition and process modelling. 
Finally, Section \ref{s:conclusions} outlines the conclusions and further research directions.
 
  %that requires of inductive techniques.  %Something that humans can do naturally and easily, such as identifying what is required to complete a task (i.e, actions, objects,intermediate states) with just a couple of examples, for a machine is a real challenge of abstraction and generalisation.


==> sections/old_introductions/introduction_v1.tex <==
\section{Introduction v1}

During the last decades, humans have tried to make possible the idea that a computer would be able to learn a monotonous task for helping humans in their daily lives. Notwithstanding the astonishing breakthrough in the field of machine learning and artificial intelligence, many tasks will take several years to make possible their automation. In this manner, humans are still indispensable in complex tasks that require appropriate use of abstract knowledge, a capability of interaction with the surrounding environment, or handling of uncertainty.  Nevertheless, there is a wide range of examples where an AI agent assists in carrying out a task and achieving a goal. This is a reality that assistive systems are becoming more important in our society and their impact on daily living for many people is increasing every day. By using the current technology, it is, therefore, possible to conceive several intelligent tools that help humans to learn to supervise and complete their tasks more efficiently.

In this sense, we pursue systems that are able to learn a task by observing a few meaningful demonstrations. This means automated assistants that, after the observation of how an expert performs a task, are able to supervise whether other humans are performing this task correctly, also by observation. We will refer to this as “supervision by observation”. This process of pervasive monitoring is made up of two sequential phases. The first one involves the knowledge acquisition by the system from observed examples and a high-level description of the task, in natural language. The second phase is carried out when the system monitors the task performed by another human how has to be supervised. More precisely, the system monitors new sequences of events and generalises them to extract the high-level meaning, which is compared with the intended high-level description of the task. Thus, the supervision agent will be capable to produce informative feedback through the supervision process. To demonstrate the potentiality of the new paradigm of supervision by observation, we will use one application domain where the technology to develop will significantly advance the current state of the art: Minimally Invasive Surgery (MIS).

In previous work, we had remarkable steps forward in this purpose. In a first instance, in [ref] we showed that it is possible to acquire new knowledge from one example by using abduction and then it can be used to recognize behaviours in different executions of the same task. Afterwards, we applied an innovative text mining technique (Text2HBM) for generating the situation model from a natural language description of several tasks. These models provided an on-fly ontology with the allowed actions and objects that will take place during the monitored performance [ref]. Eventually, in [ref], we outlined our approach for the Event Detection component, depicting the computer vision and machine learning techniques for low-level detection along the supervision. As an output of this component, we gathered a sequence of events that represent the action and movements of the human. The analysis of these sequences will be critical for the knowledge acquisition by the system. However, how to get the general planning of a task through a few example sequences?

Due to the fact that every activity has a specific idiosyncrasy, it becomes necessary the study of these sequences in a sufficiently abstract manner to skip the superfluous details. In this way, graph analysis provides multiple features to extract meaningful information from connected structures such as a sequence of steps does. Thus, some noteworthy fields such as bioinformatics [ref], social-network analysis [ref], computer vision [ref] and image processing [ref] have taken advantage of these capabilities. Subgraph finding, for instance, enables us to discover recurrent patterns that are hidden in a set of graphs [ref]. In turn, graph comparison is used to group similar graphs into clusters applying a similarity criterion [ref]. Despite the fact that these features are powerful, they are computationally expensive, as the size of the graph grows (NP-hard). Many researches during last decade have provided a wide range of kernels to address this problem.

In this paper, we propose a method to aggregate, filter and generalise the sequences of actions generated by surgeons while they are practising several MIS exercises. As a result, we are capable to obtain a set of candidate sequences with the common Minimum Sequence of Actions (MSA) that define the analysed tasks. By taking advantage of graph theory, we have developed three algorithms to carry out this process.

The rest of the paper is comprised in the following way. In Section “Related Work”, we summarise some relevant works regarding this topic. Later, we outline our method for generalising the sequences of actions, depicting the developed algorithms for this purpose. Then, in the “Experiments” section, we detail the configuration of our experimentation setting, followed by “Results and Discussion” section with the outcome of the experimental section and the analysis of the strengths and weaknesses of our approach. Finally, we conclude the paper with the paper conclusions and future work.


==> sections/old_introductions/introduction_v2.tex <==
%\sidenoteDavid{Draft text}
\section{Introduction v2}
% David: Maybe this is too general :/
% David: this is an idea for the "motivational" example about of how people learn by obsevation.
\textcolor{orange}{
Whether we were looking someone performing an activity for our first time, say, cooking a dish; we would realise what actions are taking place and, more important, which one follow each other to reach the goal. After a few observations of this task, we would be able to recognise what steps are prevailing to success, while others, in contrast, are just unusual or infrequent. At the end, we were able to assert the approximated flow to perform that activity. Although the previous process was something natural for the human learning, it currently represents an incredible drawback to machines. It also seems clear that humans take the advantage of the previous knowledge and context understanding to complete the missing information. Conversely, this is something that an AI agent lacks by default unless some background knowledge is provided by a human.}

% David: I have to adapt this part 
\textcolor{orange}{
In this sense, we pursue systems that are able to learn a task by observing a few meaningful demonstrations. This means automated assistants that, after the observation of how an expert performs a task, are able to supervise whether other humans are performing this task correctly, also by observation. We will refer to this as “supervision by observation”. This process of pervasive monitoring is made up of two sequential phases. The first one involves the knowledge acquisition by the system from observed examples and a high-level description of the task, in natural language. The second phase is carry out when the system monitors the task performed by other human who has to be supervised. More precisely, the system monitors new sequences of events and generalises them to extract the high-level meaning, which is compared with the intended high-level description of the task. Thus, the supervision agent will be capable to produce an informative feedback through the supervision process. To demonstrate the potentiality of the new paradigm of supervision by observation, we will use one application domain where the technology to develop will significantly advance the current state of the art: Minimally Invasive Surgery (MIS).}

\textcolor{red}{FALTARÍA ESPECIFICAR EN QUÉ PARTE SE VA A CENTRAR EL ARTÍCULO. Nos vamos a centrar en la parte de aprendizaje y, en concreto, la parte de "aprender" todas las formas de realizar una tarea de forma correcta a partir de unos pocos ejemplos introducidos por los expertos. Además, habría que resaltar que el método de aprendizaje no estaría limitado a la fase de entrenamiento sino que se podría seguir durante toda la vida útil del sistema mientras le sigan llegando ejecucciones correctas llevadas a cabo por el sistema. Además, el aprender todas las formas de realizar correctamente una tarea también es algo que diferencia nuestro sistema de uno de automatización de tareas. En la automatización basta con aprender como ejecutar una tarea correctamente. Además, precisa de aprender todos los detalles de esa tarea. En Supervisión, hay que aprender todas las formas de llevar a cabo una tarea pero no hace falta aprender el detalle, basta con aprender los pasos clave para conseguir llevar a cabo la tarea con éxito. El aprender todas las formas de realizar la tarea y diferenciar entre los pasos clave y los superfluos son los objetivos del trabajo que se presenta en este paper.}

==> sections/old_introductions/introduction_v3.tex <==
%\textcolor{blue}{
%\begin{itemize}
%Outline: \\
%    \item Sistemas de supervisión automática basados en visión por ordenador (Presentación de este dominio)\\
%    \item Beneficios potenciales de un sistema de supervisión de este tipo \\
 %   \item Requisitos de un sistemas de supervisión automático\\
%    \item Limitaciones de los sistemas actuales basados en automatización\\
%    \item Alternativa -> SUPERVASION\\
 %   \item Punto actual y motivación del nuevo desarrollo
 %   \item Outline del artículo.
%\end{itemize}
%}
\section{Introduction v3}
%\sidenoteDavid{Draft text}

In the last decade, automatic supervision system by computer vision has been an active research area with applications in public and industrial services. Domains such as surveillance, smart environments or surgery, have been benefited by the deployment of these systems for detecting events of risk or assisting people during their task accomplishment. In this context, a low-level reasoning of the user's actions it is not suitable due to this makes the system to be prone to noise from observation layer, totally domain dependent, and data greedy. Thus, it becomes necessary an abstract reasoning throughout the user task for providing a reliable supervision and assistance. To that end the system should be capable not only of recognising the current user's state, but also the potential future actions and the goal that he or she pursues. In short, the possible plans that lead the user to meet the task fulfilment. 

In Plan Recognition (PR), a plan is defined as a sequence of actions starting from an initial state to a goal state, where one assumes that user actively tries to achieve the goal \cite{kruger2016activity}. As can be seen, there rises several challenges to be addressed for modelling the latter in a computerised manner. For instance, human tasks can be seen as a sequences of activities with a hierarchical structure that goes from the low-level data to the high-level concepts that bestow semantic on to the activity relations. Tasks are intelligible to humans at some of the levels of the hierarchy, especially at the abstract ones. Therefore, several mappings are possible at different levels \cite{aggarwal2011human}. Furthermore, given a task, the exact representation of all possible states that can be posed is computationally infeasible. Approximative methods have been proposed for simplifying the state space search by using different filtering methods. Finally, there is required a learning phase where the system acquires the knowledge about the prevailing ways for performing a task. Issues such as data scarcity, ``cold start'' problem, noise handling and divergence between sequence instances should be overhauled.

A traditional way to address the task representation and reasoning has been under the vision of a data-driven approach. Specifically, it is formed by the combination of a top-down methodology for modelling the plan space, where the possible activity transitions (flow) are defined by a programmer, and a probabilistic and statistical method for learning the scenarios. The common models are based on supervised machine learning techniques, such as Hidden Markov Models (HMMs) and dynamic and naive Bayes networks \cite{chen2012sensor}. Even though this approach has demonstrated its utility on countless occasions for task automation, there exists several drawbacks when it is used for automating the supervision in complex environments. First of all, these techniques are highly-dependent on human intervention for providing all possible workflows as a initial step. This fact can entails an unnecessary waste of time and effort in the case of many of them were not supported by observed examples. In other words, the system may be forced to manage a range of superfluous details that they are not meaningful for representing the task. Conversely, and with regards to the knowledge acquisition, the training step is a quite rigid process inside the established life cycle in machine learning. In this manner, once the system is trained, there is not considered an specific process for learning new information whether several unseen and relevant instances arrive during the supervision. Furthermore, they still requiring large datasets for training, with the additional limitations that it means in domains without enough data. All of this will make the approach very narrowed in terms of versatility, reusability and knowledge generalisation. 

Given that an effective supervision needs to know not only how is the ``right'' manner to perform a task, just as automation does, but also the different ways, equally valid, that lead the task to the success. Apart from this, if the context involves a high complexity, and the number of examples for learning is limited, the supervision is only feasible with a strong bias. As in humans, this bias is represented by the prior knowledge about the domain and environment. Taking into account these constraints, and as an alternative to the data-driven approaches, we proposed in \cite{monserrat2016knowledge} a knowledge-based supervision framework that fills these gaps by learning from a few meaningful demonstrations performed by experts, and a background domain knowledge provided in logical format. Even though a task can be performed in different ways, we believe the task role underlies within them and it must be present in each relevant observation. Thus, there exists the possibility to capture that essence from several but ``rich'' examples.  New methods are required for bringing the different plan executions together, mining the dominant manners, and filtering the main steps from the superfluous one. Only in this manner we will provide both the key steps and the diversity of performing forms to the system. 

%%%%%%% Provisional %%%%%%%%
In order to address these challenges, in this paper we propose a novel method for mining representative plans from a set of activity flows. \textcolor{red}{Completar!!} The potentiality of this approach will be tested by it application to automatic skill supervision in minimally invasive surgery. 

The rest of this paper is organised in the following manner. Section 2 reviews the background aligned with the automatic supervision, plan mining and surgical tasks domain. Section 3 formalises the problem and some basic definitions, then we presents our algorithm for mining valid and common task flows. Then, Section 4 presents the experimental setup for evaluation and results, followed by Section 5 with the corresponding discussion. Finally, Section 6 depicts our conclusions and further research directions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/old_introductions/introduction_v4.tex <==
%\section{Introduction}
%\todo[inline, color=green!40]{
%Outline: \\
%- Sistemas de supervisión automática basados en visión por ordenador (Presentación de este dominio)\\
%- Beneficios potenciales de un sistema de supervisión de este tipo \\
%- Requisitos de un sistemas de supervisión automático\\
%- Limitaciones de los sistemas actuales basados en automatización\\
%- Alternativa -> SUPERVASION\\
%- Punto actual y motivación del nuevo desarrollo
%- Outline del artículo.
%}

\section{Introduction v4}
Despite humans are still indispensable for developing complex tasks where automation is not feasible yet, supervision systems have arisen as a suitable alternative. In contexts where an appropriate use of abstract knowledge or an interaction capability with the surrounding environment are required by an operator or apprentice, those systems may be able to supervise whether a human is performing the task correctly, detect deviations from the established plan, and advice him or her in real time if that were the case. A technology of this kind is specially applicable to supervise work stations under a well-defined workflow or strict protocol, or also for training environment where a continuous monitoring and feedback is the basis for a correct learning of procedures. These systems has been enhanced (mainly) by advances in Activity Recognition (AR) \cite{sukthankar2014plan} \textcolor{blue}{Buscar en la tesis de Kruger qué cita cuando se refiere a AR}. %\cite{huang2010flexible} \textcolor{blue}{meter citas}. 
Over the past decades, AR research area has provided a wide range of approaches to recognise human activities in multiple domains, such as industry \cite{marinho2017preliminary} \cite{maekawa2016toward} \cite{roitberg2015multimodal} \cite{wu2012automated} \cite{petrovic2010context},  surveillance \cite{batchuluun2017fuzzy} \cite{kardas2017svas} \cite{mabrouk2017abnormal} \cite{hu2013incremental} \cite{zin2010markov} \cite{ran2010applications}, smart environments and daily-living assistance \cite{chernbumroong2013elderly} \cite{banos2012daily} \cite{ayase2008method} \cite{camacho2014ontology} \cite{brdiczka2009learning} \cite{hoey2010automated}  \cite{yordanova2017s} or medicine and health-care  \cite{sanchez2008activity} \cite{corchado2010using} \cite{negin2018praxis} \cite{nakawala2017development} \cite{soutschek_measurement_2010} \cite{hein_saphire_nodate} \cite{dosis2005synchronized} \cite{ghali2003object} \cite{yordanova2017situation}. The socioeconomic impact derived from the latter has been remarkable for many human daily situations, allowing the instant detection of a human mistake that can cause a risky situation, or assisting people during their task accomplishment by providing meaningful and comprehensible feedback. 

These automatic supervisors usually work in two sequential phases. First of all, these systems must learn the essence of how one task is done from examples provided by experts. Once all the ways of performing a task are learnt, the system should be able to supervise the task executed by an apprentice by comparing her execution with the ones learnt in the first phase. Therefore, considering that there are different ways of correctly executing one task, the system must learn all of them to perform a proper supervision. In this way, the system should be capable not only of recognising the current user’s state but also potential future actions and the goal that he or she pursues. In short, the possible plans that lead the user to meet the task fulfilment. In this context, Plan Recognition \cite{sukthankar2014plan} \textcolor{blue}{[meter citas recogidas de la tesis de Kruger sobre reconocimiento de planes]} plays a fundamental role in the learning phase (the first one mentioned before) in order to generalise the execution of a given task.

It is a fact that for an effective supervision, it is needed to know all the different ways that lead the task to success and, in many cases, they lack of a high number of examples that can be used during the learning phase. In this context, a low-level reasoning of the user’s actions is not suitable because this makes the system to be prone to noise from the observation layer, they are totally domain dependent and they use information of low level events that lack of enough high level information to actually help in the development of the task \cite{chen2012sensor}. Thus, it becomes necessary an abstract reasoning throughout the user task for providing a reliable supervision and assistance. In domains where lack of data is a reality, the automatic supervision must go away from classical machine learning techniques and use some other methods that allow the introduction of strong bias that is represented by the prior knowledge about the domain and environment. In short, the learning process have to extract more from less. Learning from few example is possible if the search space is sufficiently constrained. Then, given the fact the task is known, the challenge there is to identify the space of correct manners (i.e., the search space for the plans) that could achieve the task goal. \textcolor{blue}{In our case, the previous bias lies in the assumption that each example is performed by a skilled expert on the matter, which lend it to be considered as the correct way that must be followed to perform the task under supervision in the proper way. }  

%In this context, 
The authors of this paper proposed in \cite{monserrat2016knowledge} a knowledge-based supervision framework that fills the mentioned gaps by learning from a few but meaningful demonstrations performed by experts, and a background domain knowledge provided in logical format. From this work we observed that, even though a task can be performed in different ways, the general way of developing this task underlies them and must be present in each relevant observation. Therefore, there is the possibility of capturing that essence from several but ``rich'' examples. Nonetheless, in the transition from the observed information to the logical knowledge acquisition is still necessary to design mechanisms, not only to provide the task boundaries, but also to identify an optimal representation of them. This would provide a good initial guess about which activities, together with their relationships, compound the route map where the task steps must flow for its proper fulfilment. Then, new methods are required to join the different executions, mining the dominant ways, and filter the main steps from the superfluous ones. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.  

In order to address those challenges, the contribution of this paper is two-fold: (1) we present a novel approach to mine Plan Space Models \textcolor{blue}{[quizá denominarlos como (PSM) o Plan Space Graphs]} from a set of labelled sequence of activities until all the examples are represented by at least one of those models. As an outcome, we get compact (we use ``compact'' in this paper to mean a small size). plan spaces where the main activities and their relationships are kept on it. This allows us to filter the superfluous information that is not strictly necessary to learn the task. This is a self-driven method, therefore any parameter, with the exception of the input dataset, must be adjusted or provided for; (2) we study the representativeness of those models according to new instances unseen by the model. For this purpose, we use several state-of-the-art  metrics from graph theory domain to measure the similarities between a PSM and a given plan instance. All this will be enable us to take a further step towards a real automation of the learning phase along the supervision process. Furthermore, our approach makes it possible to deal with the lack of examples and the divergence of manners to perform a task. The potentiality of this method will be tested in one domain characterised by the prior handicaps, the automatic skill supervision in surgical training tasks.

% •	Recognise sequences of gestures that are new to the system.
% •	Recognise repetitions.
% •	Detect boundaries of a task.
% •	Identify the optimal representation for a certain task.

% How to get the general planning of a task through a few example sequences?
% How to avoid/reduce the noisy transition between actions of the sequences?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Idea alternativa para el siguiente párrafo sacada del Explora %

% Fewer supervised reference procedures. One of the problems of automated supervision and evaluation of novice surgeons is that we usually have just one correct reference procedure (or at most a few) to compare with, as this requires time from experts. Obviously, the sequence of gestures performed by each novice surgeon, even if they are correct, will not be exactly the same as the sequence that we have recorded from the expert. As a result, we need to generalise the reference procedure to cover good performances and detect wrong ones. Only by proper expression of the constraints and rules that surgeons have into their background knowledge and, again, a more abstract representation, 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Poor technical skill in surgery is associated with severe adverse or even tragic implications after surgical intervention \cite{mishra2008influence}. Thus, novice surgeons develop and refine their surgical dexterities through a wide sort of training tasks under the couching of expert surgeons \cite{soper2008mastery}. %Supervision in this context is mainly focused on centric scenarios where surgical tool movement is a key element. 
The automated supervision in this context is highly biased by two factors: expert surgeon's %expertise 
idiosyncrasy and data scarcity, being necessary to find methods to deal with both if we envisages learning from a few correct reference procedures. Several approaches have tried to learn those tasks by using 
Markov structure of a surgical task and low-level motion data \cite{varadarajan2009data} \cite{tao2012sparse} \cite{lin2005automatic} \cite{reiley2008automatic}, being penalised by the previous facts as shown  the results of \cite{ahmidi2017dataset}. Furthermore, this vision makes it difficult to capture the intention and meaning of a sequence of gestures by an expert surgeon a more abstract representation of gestures is required, which is much closer to the surgeon's expertise, such as `clamp tissue from an organ', `make a knot', `separate two tissues' or `remove a spot from a tissue'. On the other hand, the sequence of gestures performed by each novice surgeon, even if they are correct, will not be exactly the same as the sequence that we have recorded from the expert. As a result, we need to generalise the reference procedure to cover good performances and detect wrong ones. Only by proper expression of the constraints and rules that surgeons have into their background knowledge and, again, a more abstract representation, can an supervision system extract the essential steps of what the procedure requires. 



% Sobre los dos problemas que tratamos: estilos y pocos datos.

% and/or 2) for dexterous and mentored tasks, such as surgical activities, individual subjects develop certain styles, resembling their mentors. Therefore, activities performed by expert individuals may differ stylewise from those performed by other experts, a potential source of variability even across expert task executions.

% According to the former, even the simplest surgical task requires a high level of dexterity and long training hours on a surgery simulator to develop it \cite{kothari2002training}. When the complexity of the task raise, the more additional activities are needed to perform it \cite{cao1996task}. In this situation, some of them can be considered as a supportive to ease the following step of the surgery task. The lack of experience, for instance, leads to use more of those activities than strictly required. Indeed, as the surgeon's expertise grows up, these surgical manoeuvres tend to be less used \cite{vedula2016analysis}. However, radically different is the fact that some skilled surgeons develop a particular manner to undertake the training task. This entails that some of these supportive activities can be embedded within the typical surgeon's performance workflow. Therefore, it is likely that two activity sequences, maybe from two different surgeons, be perfectly valid, being one significantly different to the other. On the other hand, this domain is penalised by the inherent difficulties to record datasets in comparison to others AR research areas. This is mainly caused by the high cost of the surgical simulators \cite{bric2016current} and the limited availability of access to skilled surgeons to record examples with enough quality. 


%%%%%%% Provisional %%%%%%%%


% We will use a common surgical task as a test-bed for our approach. Suturing task is a common training routine that entails some of the most challenging manoeuvres with the suturing needle, such as grasping or dot passing. These difficult actions must be repeated \emph{k} times in a suturing cycle, which raises the possibility of divergence between each iteration inside the same task. 

\textcolor{blue}{completar} 

The rest of this paper is organised in the following manner. Section 2 reviews the background aligned with the automatic supervision, plan mining and surgical tasks domain. Section 3 formalises the problem and some basic definitions, then we presents our algorithm for mining valid and common task flows. Then, Section 4 presents the experimental setup for evaluation and results, followed by Section 5 with the corresponding discussion. Finally, Section 6 depicts our conclusions and further research directions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/old_introductions/introduction_v5.tex <==
%\section{Introduction}
%\todo[inline, color=green!40]{
%%- Sistemas de supervisión automática (Presentación de este dominio)\\
%- Fases de la supervisión \\
%- Problemas existentes en dominios con pocos ejemplos y diversidad de formas de realizar una tarea.\\
%- Limitaciones de los sistemas actuales basados en datos\\
%- Alternativa -> Aprender de pocos ejemplos pero significativos.\\
%- Punto actual y motivación del nuevo desarrollo.
%- Outline del artículo.
%}
\section{Introduction v5}

Despite humans are still indispensable for developing complex tasks where automation is not feasible yet, supervision systems have arisen as a suitable alternative. In contexts where an appropriate use of abstract knowledge or an interaction capability with the surrounding environment are required by an operator or apprentice, those systems may be able to supervise whether a human is performing the task correctly, detect deviations from the established plan, and advice him or her in real time if that were the case. A technology of this kind is specially applicable to supervise jobs under a well-defined workflow or strict protocol, or also for training environment where a continuous monitoring and feedback is the basis for a correct learning of procedures. These systems has been enhanced (mainly) by advances in Activity Recognition (AR) \cite{sukthankar2014plan} %\textcolor{blue}{Buscar en la tesis de Kruger qué cita cuando se refiere a AR}. %\cite{huang2010flexible} \textcolor{blue}{meter citas}. 
Over the past decades, AR research area has provided a wide range of approaches to recognise human activities in multiple domains, such as industry \cite{marinho2017preliminary} \cite{maekawa2016toward} \cite{roitberg2015multimodal} \cite{wu2012automated} \cite{petrovic2010context},  surveillance \cite{batchuluun2017fuzzy} \cite{kardas2017svas} \cite{mabrouk2017abnormal} \cite{hu2013incremental} \cite{zin2010markov} \cite{ran2010applications}, smart environments and daily-living assistance \cite{chernbumroong2013elderly} \cite{banos2012daily} \cite{ayase2008method} \cite{camacho2014ontology} \cite{brdiczka2009learning} \cite{hoey2010automated}  \cite{yordanova2017s} or medicine and health-care  \cite{sanchez2008activity} \cite{corchado2010using} \cite{negin2018praxis} \cite{nakawala2017development} \cite{soutschek_measurement_2010} \cite{hein_saphire_nodate} \cite{dosis2005synchronized} \cite{ghali2003object} \cite{yordanova2017situation}. The socioeconomic impact derived from automatic supervision %the latter 
would be remarkable for many human daily situations, allowing the instant detection of a human mistake that can cause a risky situation, or assisting people during their task accomplishment by providing meaningful and comprehensible feedback. 

These automatic supervisors usually work in two sequential phases. First of all, these systems must learn the essence of how one task is done from examples provided by experts. Once all the ways of performing a task are learnt, the system should be able to supervise the task executed by an apprentice by comparing her execution with the ones learnt in the first phase. Therefore, considering that there are different ways of correctly executing one task, the system must learn all of them to perform a proper supervision. In this way, the system should be capable not only of recognising the current user’s state but also potential future actions and the goal that he or she pursues. In short, the possible plans that lead the user to meet the task fulfilment. In this context, Plan Recognition (PR) \cite{sukthankar2014plan} plays a fundamental role in the learning phase (the first one mentioned before) in order to generalise the execution of a given task.

%It is a fact that for an effective supervision, it is needed to know all the different ways that lead the task to success and, in many cases, 
It is a fact that most supervision systems lack of a high number of examples to make use during the learning phase. As if this were not enough, some people perform certain activities significantly differently from the others. Training data therefore not experience enough variants of the activity patterns to create a generic model. In this context, a low-level reasoning of the user’s actions is not suitable because this makes the system to be prone to noise from the observation layer, they are totally domain dependent and they use information of low level events that lack of enough high level information to actually help in the development of the task \cite{chen2012sensor}. Thus, it becomes necessary an abstract reasoning throughout the user task for providing a reliable supervision and assistance. In domains where lack of data is a reality, 
The automatic supervision must go away from classical machine learning techniques and use some other methods that allow the introduction of strong bias that is represented by the prior knowledge about the domain and environment. In short, the learning process have to extract more from less. Learning from few example is possible if the search space is sufficiently constrained. From our point of view, this bias could be obtained from some meaningful examples performed by skilled experts on the matter, which lend it to be considered as the correct way that must be followed to perform the task under supervision in the proper way \cite{monserrat2016knowledge}.  

%In this context, 
% The authors of this paper proposed in \cite{monserrat2016knowledge} a knowledge-based supervision framework that fills the mentioned gaps by learning from a few but meaningful demonstrations performed by experts, and a background domain knowledge provided in logical format. 
Existing literature in PR \cite{yang2007learning}  \cite{yang2005learning} \cite{blythe2001integrated} \cite{benson1995inductive} \cite{wang1995learning} have shown it is possible to acquire the missing knowledge concerning tasks by learning from plan observations. Even though a task can be performed in different ways, the general way of developing this task underlies them and must be present in each relevant observation. Therefore, there is the possibility of capturing that essence from several but ``rich'' examples. Nonetheless, in the transition from the detected information to the logical knowledge acquisition is still necessary to design mechanisms, not only to provide the task boundaries, but also to identify an optimal representation of them. This would provide a good initial guess about which activities, together with their relationships, compound the route map where the task steps must flow for its proper fulfilment. Then, given the fact the task is known, the following step is to identify the space of correct ways (i.e., the search space for the plans) that could achieve the task goal. The huge challenge is address this goal in contexts where data is lacking and the variety of perfectly valid performances is a distinguishing feature. New methods are required to join the different executions, mining the dominant ways, and filter the main steps from the superfluous ones. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.  

In order to address those challenges, the contribution of this paper is two-fold: (1) we present a novel approach to mine \FullNamePlanSpaceGraph{s} \textcolor{blue}{[quizá denominarlos como (\ShortNamePlanSpaceGraph) o Plan Space Models (PSM)]} from a set of labelled sequence of activities until all the examples are represented by at least one of those models. As an outcome, we get multiple compact (we use ``compact'' in this paper to mean a small size) plan spaces where the main activities and their relationships are kept on it. This allows us to filter the superfluous information that is not strictly necessary to learn the task%.It is a self-driven method, therefore any parameter, with the exception of the input dataset, must be adjusted or provided for
; (2) we study the representativeness of those models according to new instances unseen by the model. For this purpose, we use several state-of-the-art  metrics from graph theory domain to measure the similarities between a \ShortNamePlanSpaceGraph and a given plan instance. All this will be enable us to take a further step towards a real automation of the learning phase along the supervision process. Furthermore, our approach makes it possible to deal with the lack of examples and the divergence of ways to perform a task. The potentiality of this method will be tested in one domain characterised by the prior handicaps, the automatic skill supervision in surgical training tasks.

% •	Recognise sequences of gestures that are new to the system.
% •	Recognise repetitions.
% •	Detect boundaries of a task.
% •	Identify the optimal representation for a certain task.

% How to get the general planning of a task through a few example sequences?
% How to avoid/reduce the noisy transition between actions of the sequences?

\textcolor{blue}{[Pendiente completar cuando se tenga el paper] 
The rest of this paper is organised in the following manner. Section 2 reviews the background aligned with the automatic supervision, plan mining and surgical tasks domain. Section 3 introduce the activity data, formalises the problem and some basic definitions, then we presents our algorithm for mining valid and common task flows. Then, Section 4 presents the experimental setup for evaluation and results, followed by Section 5 with the corresponding discussion. Finally, Section 6 depicts our conclusions and further research directions.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/old_introductions/introduction_v6.tex <==
\section{Introduction v6}
Despite humans are still indispensable for developing complex tasks where automation is not feasible yet, supervision systems have arisen as a suitable alternative. In contexts where an appropriate use of abstract knowledge or an interaction capability with the surrounding environment are required by an operator or apprentice, those systems may be able to supervise whether a human is performing the task correctly, detect deviations from the established plan, and advice him or her in real time if that were the case. A technology of this kind is specially applicable to supervise jobs under a well-defined workflow or strict protocol, or also for training environments where a continuous monitoring and feedback is the basis for a correct learning of procedures. Namely, it could be seen as an automatic expert in the matter made to help in this task and ultimately to enhance itself by supervision and guidance. These systems has been strengthen (mainly) by advances in Activity Recognition (AR) \cite{sukthankar2014plan}, providing a wide range of approaches to recognise human activities in multiple domains, such as industry (\cite{marinho2017preliminary}, \cite{maekawa2016toward}%, \cite{roitberg2015multimodal}, \cite{wu2012automated}, \cite{petrovic2010context}
),  surveillance (\cite{batchuluun2017fuzzy}, \cite{kardas2017svas}, \cite{mabrouk2017abnormal}%, \cite{hu2013incremental}, \cite{zin2010markov}, \cite{ran2010applications}
), smart environments and daily-living assistance (\cite{chernbumroong2013elderly}, \cite{banos2012daily}, \cite{hoey2010automated}%\cite{ayase2008method}, \cite{camacho2014ontology}, \cite{brdiczka2009learning},  \cite{yordanova2017s}
), or medicine and health-care (\cite{sanchez2008activity}, \cite{corchado2010using}, \cite{negin2018praxis}%, \cite{nakawala2017development}, \cite{soutschek_measurement_2010}, \cite{hein_saphire_nodate}, \cite{dosis2005synchronized}, \cite{ghali2003object}, \cite{yordanova2017situation}
). The socioeconomic impact derived from automatic supervision %the latter 
would be remarkable for many human daily situations, allowing the instant detection of a human mistake at work that can cause a risky situation, or assisting people during their task accomplishment by providing meaningful and comprehensible feedback. 

These automatic supervisors usually work in two sequential phases. First of all, such systems must learn the essence of how one task should be done from examples provided by experts. Secondly, once all the ways of performing a task are learnt, the system should be able to supervise the task executed by an apprentice by comparing her execution with the ones learnt in the first phase. Therefore, considering that there are different ways of correctly executing one task, the system must learn all of them to perform a proper supervision. In this way, the system should be capable not only of recognising the current user’s state but also potential future actions and the goal that he or she pursues. In short, the possible plans that lead the user to meet the task fulfilment. In this context, Plan Recognition (PR) \cite{sukthankar2014plan} plays a fundamental role in the learning phase (the first one mentioned before) in order to generalise the execution of a given task.

%It is a fact that for an effective supervision, it is needed to know all the different ways that lead the task to success and, in many cases, 

Traditionally, most supervision systems show two important drawbacks: a high dependency of training data during the learning phase and a short-sighted reasoning according with the actor's actions and the ongoing task. On one hand, it is required extensive amounts of data for training the recognition algorithms. Despite the proliferation of datasets with contextualised human activities in a range of situations, there are many more where the specificity of the entailed actions make that information useless. Therefore, new data must be gathered and annotated, with the subsequent economic and time-consuming effort which it implies. And if this were not enough, in some human routines, people perform certain activities significantly differently from the others; training data may therefore not express enough variants of the users plans to create a general model. On the other hand, reasoning without enough abstraction (i.e., low-level reasoning) about user’s actions is not suitable to that end for several reasons. First of all, those systems tend to be more prone to noise from observation layer such as sensor data, video signal, etc. Second, they are usually designed for an specific domain application, discarding the generalisation mechanisms to ease the reusability of the acquired knowledge for other purpose. Moreover, complex activities are only recognisable at certain level of abstraction, thus a high-level reasoning in this regard enhance the capability of the system to offer valuable assistance when a skill-demanding task is being carried out by the user \cite{chen2012sensor}. %Thus, it becomes necessary an abstract reasoning throughout the user task for providing a reliable supervision and assistance. 

In domains where lack of data is a reality, automatic supervision must go away from %classical machine learning 
those data-driven techniques and use some other methods that allow the introduction of strong bias that is represented by the prior knowledge about the domain and environment. To put it simply, the learning process has to extract more from less. This challenge has characterised at length the research area of Inductive Programming (IP) \cite{gulwani2015inductive}, area where artificial intelligence, machine learning and cognitive science join together in order to learn human routines, in the form of computer programs, from several examples observations and some declarative background knowledge. IP is concerned about making expert systems learn programs automatically in situations where data become scarce. Moreover, experts knowledge can enhance significantly the system performance by introducing the domain constraints, as long as that knowledge is captured appropriately by the system. Inductive programming has been successful for repetitive task automation in other human-related application domains, such as data transformation tasks with FlashFill \cite{gulwani2011automating} or  FlashExtract \cite{gulwani2017framework} tools, or creating educational content for different subjects as logic, programming or algebra, directly from examples \cite{gulwani2014example}. Needless to say, learning a complex task from a few instances in a physical environment entails many more challenges, however, we believe this is possible if those examples are meaningful enough describing the task, an appropriate level of abstract reasoning is achieved, and the right tools and mechanisms are developed to acquired the knowledge of the experts in the matter \cite{monserrat2016knowledge}. But there is also still to bridge the gap between the observed information and the logical knowledge acquisition. Therefore, some kind of generalisation approach is required to that end; that is, put in common the different task observations, mining the dominant plans, and filter the main steps from the superfluous ones. In this regard, a refinement mechanism will also be necessary to search, in the space of possible solutions, the most accurate model according to the observed examples, even when they present little discrepancies between them, or notably different plans of performing the task.
\sidenoteDavid{No sé muy bien como meter ILP aquí. Antes lo tenía más claro (estaba en lugar de IP), pero al meter IP arriba se me ha desbarajustado. ¿Alguna idea?}

% All this In supervision contexts where data is lacking and the supervised task is skill demanding for humans Different the d Similar issue is addressed by Inductive Logic Programming (ILP) systems in order to find the most general hypothesis capable to cover the examples.  where bottom-up systems face the problem from the mor where a logical framework for inductive learning,  of developing it are sufficiently delimited for the system.

% by developing inductive refinement techniques to find the most accurate model according to the observed examples in a search space of possible manners candidates. As in Inductive Logic Programming (ILP) 

% Mechanisms to But as in other inductive learning context, a general pattern is underlying the examples and must be present in each relevant observation  inductive refinement techniques to find the an underlying representation and most accurate according to the observed examples.

% , all this in order to synthesise the task in a general representation. In  a first incursion in inductive supervision were achieved, where obtained from some meaningful examples performed by skilled experts on the matter, which lend it to be considered as the correct way that must be followed to perform the task under supervision in the proper way . Nevertheless, 
% Nevertheless, mechanism to deal with  and the search space of possible manners of developing it are sufficiently delimited for the system. In this sense, %Inductive Logic Programming (ILP) \cite{muggleton1994inductive} provides 
% some inductive refinement techniques to find the an underlying representation and most accurate according to the observed examples.

% Even though a task can be performed in different ways, we believe that a general pattern underlies them and must be present in each relevant observation. Therefore, there is still necessary to bridge the gap between the observed information to the logical knowledge acquisition with some kind of generalisation mechanism. In supervision contexts where data is lacking and the supervised task is skill demanding for humans, new methods are required to put in common different observations, mining the dominant ways, and filter the main steps from the superfluous ones.

% On the other hand, existing literature in PR (\cite{yang2007learning}, \cite{yang2005learning}, \cite{blythe2001integrated}, \cite{benson1995inductive}, \cite{wang1995learning}) have shown it is possible to acquire the missing knowledge concerning tasks by learning from plan observations. 
 % Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.   %Therefore, there is the possibility of capturing that essence from several but ``rich'' examples. Nonetheless, in supervision contexts where data is lacking and supervised task is skill demanding for humans, there still necessary to bridge the gap between the observed information to the logical knowledge acquisition with some kind of generalisation mechanism. New methods are therefore required to put in common different observations, mining the dominant ways, and filter the main steps from the superfluous ones. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.   
In order to address this generalisation challenge in human task supervision, the contribution of this paper is twofold: (1) we present a novel inductive approach to extract \FullNamePlanSpaceGraph{s} \textcolor{blue}{[quizá denominarlos como (\ShortNamePlanSpaceGraph) o Plan Space Models (PSM)]} from a set of labelled sequence of activities until all the examples are represented by at least one of those models. As an outcome, we get multiple ``compact'' (we use this term in this paper to mean a smaller size compared to the addition of individuals) plan patterns, where the main activities and their relationships are kept on it. This allows us to filter the superfluous information that is not strictly necessary to learn the task; (2) we study the coverage of those models according to new instances unseen by those patterns. For this purpose, we use several state-of-the-art metrics from graph theory domain to measure the similarities between a \ShortNamePlanSpaceGraph{} and a given plan graph instance. All this will be enable us to take a further step towards a real automation of the learning phase along the supervision process. Furthermore, our approach makes it possible to deal with the lack of examples and the divergence of ways to perform a skill-demanding task. The potentiality of this method will be tested in one domain characterised by the prior handicaps, that is the automatic %skill 
supervision in surgical training tasks. 

% •	Recognise sequences of gestures that are new to the system.
% •	Recognise repetitions.
% •	Detect boundaries of a task.
% •	Identify the optimal representation for a certain task.

% How to get the general planning of a task through a few example sequences?
% How to avoid/reduce the noisy transition between actions of the sequences?

\textcolor{blue}{[Pendiente completar cuando se tenga el paper] 
The rest of this paper is organised in the following manner. Section 2 reviews the background aligned with the automatic supervision, plan mining and surgical tasks domain. Section 3 introduce the activity data, formalises the problem and some basic definitions, then we presents our algorithm for mining valid and common task flows. Then, Section 4 presents the experimental setup for evaluation and results, followed by Section 5 with the corresponding discussion. Finally, Section 6 depicts our conclusions and further research directions.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/old_introductions/introduction_v7.tex <==
\section{Introducción v7} %\sidenoteDavid{Versión nueva de la introducción (versión antigua enviada por email)}

Automatic supervision of monotonous tasks could be a reasonable alternative to their automation, making the human performance more reliable and efficient because of the constant monitoring at a considerably reduced cost. This supervision would care about whether the operators would be developing the task correctly, detecting deviations from the established plans, and advising them in real time providing meaningful feedback. As a result, an automatic supervisor could prevent some tasks from being spoilt, i.e., leading to suboptimal results or implying a potential risk due to human mistakes. Moreover, constant supervision could enhance some jobs by supporting the apprentices with useful feedback and guidance in the early steps. The latter is of relevance in certain jobs where poor technical skills during the instructional stage have been associated with adverse outcomes or even tragic consequences \cite{birkmeyer2013surgical}.

Before performing the supervision, the supervisor system will need to learn the essence of how one task should be done, coded by a programmer or learnt from (potentially few) examples and procedures provided by experts. However, manual coding is discarded as a solution since the supervision process is expected to be completely automatic. Otherwise, this would represent a high effort to define, or in extreme case, to directly program all the possible plans of performing the task, as well as updating them when new methods would appear over time. It is also envisioned to be general, transversal and pervasive enough to be tuned to multiple domains, independently of the amount of available examples and the different ways in which a task can be performed. Considering that there may be different ways of correcting a possible wrong action, the system must be able to generalise in such a way that goes beyond particular cases and `understand' the intermediate goals of a task. 

Traditionally, similar learning processes have been addressed in Activity Recognition (AR) \cite{sukthankar2014plan}, using both data-based approaches and knowledge-based approaches \cite{chen2012sensor}. To date, data-based approaches have been the predominant way to generalise task models, relying on an intensive use of pre-existent data from users’ activities. However, these approaches are no suitable for domains where there is not enough data. An alternative way (i.e., knowledge-based approaches) implies to take advantage of the previous knowledge about the domain as a resource to generalise or learn a procedure. However, despite similarities with other applications in AR, the learning process for supervision must be focused not on knowing one possible way to perform one task, but all the correct ways to carry it out. It means to learn all the different plans to perform that task. This learning process could be narrowed by using the experts' experience and background in order to record those meaningful demonstrations of how this task should be performed. As this requires time and effort from experts, there is expected a little correct reference examples to learn from. For this reason, we aim to provide a generalisation method to automate the extraction of the essential workflows of activities (i.e., patterns) from a few expert plan executions according to a task to be supervised. In this sense, there are not much researches focusing on context with a lack of observations and a high diversity of plans to be learned by the system.

In this paper, we present a novel approach to address this generalisation problem by using a method based on graph theory. Our approach allows extracting predominant patterns from a set of plan performances expressed as annotated sequences of activities. First, we propose a formal framework to represent the sequences as directed graphs of activities, where nodes represent the types of activities and the directed edges represent the transitions. Some characteristics of human tasks, such as step cycles, can be expressed by using graphs better than annotated sequences. Moreover, graphs are a common notation used in the workflow analysis (\citep{van2004workflow} with applications in bioinformatics \citep{yan2005mining}, social-network analysis \citep{carrington2005models} or web navigation \citep{papadimitriou2010web}. Then, we propose an algorithm that operates over the graphs for mining the underlying patterns according with the edge popularity in the set of examples.  This means that the popular steps remain in the pattern as long as the superfluous information is filtered from them because it is not strictly necessary to learn the essence of the task. The algorithm also ensure the validity of each pattern, as a complete representation of the task, at the same time that all examples are covered by at least one pattern.  These make our approach suitable to provide the supervision system with all the valid ways, and also capable of extracting more from less when a few plan examples are available to carry out the learning process. As far as we know this is the first approach that proposes the combination of graphs to represent plans and an inductive method for providing the essential knowledge about how the task should be performed to a knowledge-based supervision system. With this purpose, we will test the potentiality of this method in one domain characterised by the rich experts’ experience and background and the (potentially) lack of recorded examples: the automatic skill supervision in surgical training tasks.

==> sections/old_introductions/introduction_v8.tex <==
\section{Introducción v8} 

In this paper, we propose a new method based on Process Mining and Inductive Programming to learn process models for posterior applications in automatic supervision systems. Automatic supervision of monotonous and/or complex processes could be a reasonable alternative to their automation, making the human performance more reliable and efficient because of the constant monitoring at a considerably reduced cost. This supervision would care about whether the operators would be developing the process correctly, detecting deviations from the established models of the process, and advising them in real-time because deviations of the model or by suggesting activities to accomplish the goals of the process (meaningful feedback). As a result, an automatic supervisor could prevent some processes from being spoilt, i.e., leading to suboptimal results or implying a potential risk due to human mistakes \cite{birkmeyer2013surgical}. 

Before performing the supervision, the supervisor system will need to learn the essence of how one process should be done, coded by a programmer or learnt automatically from examples and procedures provided by experts. Manual coding is time-consuming, little versatile and prone to obsolescence. Besides, it requires a big effort to define, or in extreme case, to directly program all the possible models of performing a process, as well as updating them when new models appear over time. On the other hand, a real automatic supervisor must be general, transversal and pervasive enough to be tuned to multiple domains. Moreover, the number of available examples use to be limited and the system must learn the different ways in which a process can be performed to carry out a correct supervision. 

Traditionally, similar learning processes have been addressed in Activity Recognition (AR) \cite{sukthankar2014plan}, using both data-based approaches and knowledge-based approaches \cite{chen2012sensor}. To date, data-based approaches have been the predominant way to generalise task models, relying on an intensive use of pre-existent data from users’ activities. However, these approaches are not suitable for domains where there is not enough data. An alternative way (i.e., knowledge-based approaches) implies to take advantage of the previous knowledge (bias) about the domain as a resource to generalise or learn a procedure. However, they use to be limited to only learn one possible way of performing a task and although the models learned are simple and plausible, they do not ensure that they are feasible. Besides, in some cases it is necessary to define the structure of the task to be learned previously \cite{hoey2010automated}.

In this paper, we aim to provide a generalisation method to automate the extraction of the essential workflows of activities (i.e., process models) from a few expert examples executions according to a task to be supervised that tries to overcome the limitations of the data-based and knowledge-based models. This is a novel approach to address this generalisation problem by using a method based on process mining techniques \cite{van2016process}, Inductive Programming and graph theory. The goal of this work is to learn the predominant process models (the backbone of the process \cite{yang2017medical}) from a set of positive examples of process performances annotated as event logs. These learned models will only contain the essential activities that will allow finishing the supervised process successfully. To build the models, we use Dependency Graphs (\cite{van2004workflow}, \cite{yan2005mining}, \cite{carrington2005models}, \cite {papadimitriou2010web}) that is one typical representation of process models with two advantages: they are easily understandable and allow filtering of non-essential activities \cite{van2016process}. One activity is considered non-essential if its execution is not necessary to finish the process correctly. The algorithm also ensures the validity of each model, as a complete representation of the process, and the feasibility of it by checking that, at least, one training example contains this model.  Finally, we have analysed the generalisation, simplicity and fitting properties of the resulting models \cite{van2016process}. 

As far as we know this is the first approach that proposes the combination of Dependency Graphs and an inductive method for process modelling in a knowledge-based supervision system. To analyse the applicability of the model, we have tested the potentiality of this method in a very challenging environment that considers all the mentioned requirements: the automatic skill supervision in surgical training tasks.



%%%%%%%%%%%% Versión antigua con Comentarios Jose %%%%%%%%%%%%

% Today, there are many human tasks whose automation is not possible yet, despite being repetitive. The automatic supervision of these tasks has arisen as a suitable step for making them more reliable and efficient, in the interim of making them fully automated. Also, supervision and overseeing may be key for contexts where other automated systems are being used, but still not very reliable. 
% %Despite the human interaction is still indispensable to perform such tasks, a  system could assist the human in the development of the task. In this sense, that system, as 
% An automated supervisor would be able to monitor whether operators are performing the task correctly, detect deviations from the established plans, and advice them in real time %, if that were the case, 
% with meaningful feedback. \sidenoteJose{A partir de aqui se repite lo mismo una y otra vez. Reescribo}Automated supervision could have a significant effect on two important spheres. On one hand, some tasks may be easily spoilt, may lead to suboptimal results or imply a potential risk by a human mistake. The supervisor system could trace the operator activities and spot the deviations from the expected performance, %. The same applies to those jobs subject to pre-established 
% workflow or protocol. %, where automated supervision would make it more secure. 
% On the other hand, humans learn some tasks more efficiently if they have continuous supervision and get meaningful feedback, but this overseeing (from an expert or a teacher) is usually expensive. Hence, the acquisition of new skills in training environments would be enhanced through systems performing automated supervision and useful feedback. Indeed, poor technical skills have been associated with adverse outcomes or even tragic consequences \cite{birkmeyer2013surgical}. These two stages (training and operation) are directly connected. The better training is through intensive monitoring and feedback the less prone to errors the operators will be. This has been shown % at is why in some domains such as surgery, it is foreseen that those systems can be potentially beneficial to improve the  
% in surgical/interventional care \cite{vedula2017surgical}.  \sidenoteJose{De nuevo nos repetimos un montón en lo que queda.} In some educational contexts, the traditional model of teaching skills relies on supervision and demonstration by experts in the matter.This method has traditionally suffered important limitations, such as limited access to realistic test beds or the availability of experts’ time to give immediate feedback and guidance during each exercise. Automatic supervisors, as coaching systems, would be an alternative to enable inexperienced trainees to learn without a continuous human expert supervision. Previously, these systems should assimilate the experts knowledge in order to provide an effective assistance and supervision. \sidenoteDavid{Nuevo}

%%%%%%%%%%%%%%%%%
% Version antigua
%%%%%%%%%%%%%%%%%
% \textcolor{blue}{Despite humans are still indispensable to develop complex tasks whose automation is not feasible yet, supervision systems have arisen as a suitable alternative to automatically assist humans when they are performing those tasks.} \sidenoteDavid{Lo he reescrito, ¿mejor así?}\sidenoteMj{rehacer la frase siguiente}In contexts where an appropriate use of abstract knowledge or an interaction capability with the surrounding environment are required by an operator or apprentice, those systems may be able to supervise whether a human is performing the task correctly, detect deviations from the established plan, and advice him or her in real time if that were the case. The training of new skills and the human errors during their execution could entail a high cost that could be reduced by automated supervision systems indicating when, where and how a protocol error takes place, in a comprehensible way for the user or the professional. \textcolor{blue}{This technology is specially applicable to supervise jobs under a well-defined workflow or strict protocol, or also for training environments where a continuous monitoring and feedback is the basis for a correct learning of procedures.}\sidenoteDavid{He usado esta frase del Explora. Creo que explica mejor la motivación de la supervisión automática} \sidenoteMj{rehacer la frase siguiente}Namely, it could be seen as an automatic expert in the matter made to help in this task and ultimately to enhance itself by supervision and guidance. These systems has been strengthen (mainly) by advances in the Activity Recognition (AR) field \cite{sukthankar2014plan}, which have provided with a wide range of approaches to recognise human activities in multiple domains, such as industry (\cite{marinho2017preliminary}, \cite{maekawa2016toward}%, \cite{roitberg2015multimodal}, \cite{wu2012automated}, \cite{petrovic2010context}
% ),  surveillance (\cite{batchuluun2017fuzzy}, \cite{kardas2017svas}, \cite{mabrouk2017abnormal}%, \cite{hu2013incremental}, \cite{zin2010markov}, \cite{ran2010applications}
% ), smart environments and daily-living assistance (\cite{chernbumroong2013elderly}, \cite{banos2012daily}, \cite{hoey2010automated}%\cite{ayase2008method}, \cite{camacho2014ontology}, \cite{brdiczka2009learning},  \cite{yordanova2017s}
% ), or medicine and health-care (\cite{sanchez2008activity}, \cite{corchado2010using}, \cite{negin2018praxis}%, \cite{nakawala2017development}, \cite{soutschek_measurement_2010}, \cite{hein_saphire_nodate}, \cite{dosis2005synchronized}, \cite{ghali2003object}, \cite{yordanova2017situation}
% ). The socioeconomic impact derived from automatic supervision %the latter 
% would be remarkable for many human daily situations, allowing the instant detection of a human mistake at work that can cause a risky situation, or assisting people during their task accomplishment by providing meaningful and comprehensible feedback. 

% Automatic supervisors usually work in two sequential phases. Firstly, the systems must learn the essence of how one task should be done (i.e., a model of the task), coded by a programmer or learnt from examples and procedures provided by experts. Secondly, once the different ways of performing a task have been learnt, the system should be able to supervise the task when it is performed by a user. As the user operates, the system will compare the ongoing actions with the generalised model and will spot the discrepancies and possible amendments in real time. Considering that there may be different ways of correcting a possible wrong action, the system must be able to generalise in such a way that goes beyond particular cases and `understand' the intermediate goals of a task.\sidenoteJose{Rewritten}
%learn all of them (\sidenoteMj{lo del parentesis lo he añadido yo}or at least the most extensively used)\sidenoteDavid{Ok} to perform a proper supervision.

% The extraction of a computational task model, in a way that allows a system to conduct supervision, is a topic widely addressed in the area of Activity Recognition (AR). Applications of AR have been proposed 
% for a wide range of domains, such as industry (\cite{marinho2017preliminary}, \cite{maekawa2016toward}%, \cite{roitberg2015multimodal}, \cite{wu2012automated}, \cite{petrovic2010context}
% ),  surveillance (\cite{batchuluun2017fuzzy}, \cite{kardas2017svas}, \cite{mabrouk2017abnormal}%, \cite{hu2013incremental}, \cite{zin2010markov}, \cite{ran2010applications}
%  ), smart environments and daily-living assistance (\cite{chernbumroong2013elderly}, \cite{banos2012daily}, \cite{hoey2010automated}%\cite{ayase2008method},  \cite{brdiczka2009learning},  \cite{yordanova2017s}, \cite{camacho2014ontology}
%  ), or medicine and health-care (\cite{sanchez2008activity}, \cite{corchado2010using}, \cite{negin2018praxis}). All these applications have been motivated (mainly) by the objective of allowing computing systems to  assist humans with their tasks. 
%  \sidenoteDavid{Nuevo}\sidenoteJose{Es Activity Recognition lo mismo que Automatic Supervision? Este párrafo da a entender que sí, y tira por tierra toda la novedad que podría tener el artículo en cuanto a supervisión, y los primeros párrafos. Para mí, activity recognition es parecido pero no lo mismo. Igual estoy equivocado, pero los nombres, al menos, son muy diferentes.}
 
 %, \cite{nakawala2017development}, \cite{soutschek_measurement_2010}, \cite{hein_saphire_nodate}, \cite{dosis2005synchronized}, \cite{ghali2003object}, \cite{yordanova2017situation}
%

% \sidenoteMj{Hasta el final de este párrafo hay que revisarlo}\sidenoteDavid{La he retocado, no sé si está más clara ahora.}\textcolor{blue}{In this way, the system should be capable not only of recognising the current state of the task, but also potential user's actions and goals. In short, the possible plans that lead the user to complete the task. In this context, Plan Recognition (PR) \cite{sukthankar2014plan} plays a fundamental role in the learning phase (the first one mentioned before) in order to generalise the execution of a given task.}


%%%%%%%%%%%% Version anterior %%%%%%%%%%%%

% These automatic supervisors usually work in two sequential phases. Firstly, the systems must learn the essence of how one task should be done (i.e. a pattern) from the examples provided by experts. Secondly, once the different ways of performing a task have been learnt, the system should be able to supervise the task executed by an apprentice by comparing her execution with the patterns learnt in the first phase. Therefore, considering that there may be different ways of correctly executing one task, the system must be able to learn all of them (\sidenoteMj{lo del parentesis lo he añadido yo}or at least the most extensively used)\sidenoteDavid{Ok} to perform a proper supervision. 
% %Therefore, considering that there may be different ways of correctly executing one task, the system must learn all of them to perform a proper supervision.
% \sidenoteMj{Hasta el final de este párrafo hay que revisarlo}\sidenoteDavid{La he retocado, no sé si está más clara ahora.}\textcolor{blue}{In this way, the system should be capable not only of recognising the current state of the task, but also potential user's actions and goals. In short, the possible plans that lead the user to complete the task. In this context, Plan Recognition (PR) \cite{sukthankar2014plan} plays a fundamental role in the learning phase (the first one mentioned before) in order to generalise the execution of a given task.}
%%%%%%%%%%%%


% ref para el párrafo\cite{chen2012sensor}

% \sidenoteJose{La intro no debería pasar de dos páginas y por fin parece que llegamos a la motivación del paper.}\sidenoteJose{Y párrafos de casi una página. Son infumables. Hay que ir al grano, sintetizar y trocear}
% According to the mechanism that is used during the learning phase, the AR approaches can be distinguished in data-based approaches and knowledge-based approaches \cite{chen2012sensor}. Traditionally, the AR applications have been dominated by the first one. These rely on an intensive use of preexistent data of users’ behaviours to obtain the task model. Data mining and machine learning techniques are used to create probabilistic or statistical models. % that are trained in a subsequent step. 
% Although both techniques are undoubtedly contrasted\sidenoteJose{lo de contrasted no creo que funcione en inglés. En cualquier caso, si funcionan no se motiva la segunda parte de la frase. ¿Tienen limitaciones, sí o no?}, the automatic supervision must go away from these methods\sidenoteJose{go away? rewrite...} if the supervision is expected to be general, transversal and pervasive enough to be tuned to multiple domains. This is motivated by several reasons. Firstly, many domains that could potentially  be benefitted by automated supervisors, are characterised by very little or sparse activity data. Although there are plenty of datasets about human activities \cite{chaquet2013survey}, this data becomes useless when the set of activities required to learn a task is specific to certain domain\sidenoteJose{No entiendo esta frase, me parece un poco contradictoria}. As a result, new data must be recorded and annotated. This process is costly and time consuming. Hence, supervision systems must learn from fewer supervised reference procedures to generalise the task. Secondly, the information necessary to make automatic supervision effective enough is not only in the observations. Tasks are more than a simple sequence of low-level actions. Indeed, they become intelligible to humans when certain level of abstraction is reached. The system should allow the definition of %deep concepts and 
% abstract knowledge in order to capture the intention and meaning of the user's actions. %ongoing performance of the user. 
% Moreover, assertive supervisors must go a step further than simple user's action recognition.\sidenoteJose{Aha... primera diferencia entre supervisor y recogniser... Pero llega muy tarde y de refilón} Deviation detection and proper feedback providing must be overhauled.\sidenoteJose{Frase no gramatical} Therefore, learning process\sidenoteJose{Learning o supervision? De todas maneras este desiderata suena a carta a los reyes} must become more cognitive and predictable, by taking more advantages of intentions, constraints, source and context of the data, rather than just looking at information as raw data. Finally, when only few observations are available, it becomes even more important to take advantage of the rich knowledge that domain experts can provide to the virtual supervisor.\sidenoteJose{Esto no se ha dicho ya? Este párrafo no acaba nunca} Appropriate learning mechanisms to acquire, codify and make use of the experts knowledge will be basis to that end.\sidenoteJose{Frase vacía} Alternatively to a data-driven approach, a knowledge-based approach makes use of those mechanisms to capture the prior knowledge in the domain to generalise the procedure to supervise.\sidenoteJose{De nuevo, esto no se ha dicho ya?} In those application domains, where automatic supervision must learn from a few reference procedures, the appropriate technology must be chosen to learn a model from incomplete information.\sidenoteJose{Frase vacía.} For that reason, an inductive approach\sidenoteJose{Qué es un "inductive approach", para mí es sinónimo de "learnign"} would be more suitable in order to fill those gaps by making the most of experts' experience and background. \sidenoteJose{En resumen, si queremos decir que nuestra propuesta recoge lo mejor de los dos mundos y consigue abstraer porque usa X, Y y Z, en vez de W, R y S no ha quedado nada claro.}
% \sidenoteDavid{Nuevo}

%%%%%%%%%%%%%%%%%
% Version antigua
%%%%%%%%%%%%%%%%%
% In those context in which the supervision system must learn from one correct reference procedure (or at most a few), automatic supervision must go away from classical machine learning and statistical modelling and use some other methods that allow the introduction of strong bias that is represented by the prior knowledge about the domain and environment.
% Though, nowadays, there are datasets with many human activities in different situations and scenarios to generate those model \cite{chaquet2013survey}, certain domain activities are so specialised that new data must be recorded and annotated. This is costly and timeconsuming. Additionally, it is a fact that people can perform certain activities significantly differently from others. Training data might not contain enough variants of the users plans to create a general model capable of expressing as many ways of performing the task as possible. This usually leads to models that are not scalable or reusable. Finally, supervising a task involves much more than a sequence of linked activities that can be derived from the data. Low-level actions makes it difficult to capture the intention and meaning of the ongoing performance of the user. 
% textcolor{red}{and a short-sighted reasoning  \sidenoteMj{la palabra reasoning tiene que explicarse. Te refieres a que los patrones no tienen en cuenta las acciones ni la tarea?} in regard to the actor's actions and the ongoing task. On one hand, most recognition algorithms require extensive amounts of training data. \sidenoteMj{las 2 frases que vienen a continuacion no se entienden}
% Although there are multiple datasets based on human activities for different situations and scenarios \cite{chaquet2013survey}, when certain tasks to be monitored entail a set of very specific activities, make the previous dataset useless to train a model for that purpose. Therefore, new data must be gathered and annotated, with the subsequent economic and time-consuming effort which it implies. Additionally, as in some human routines some people can perform certain activities significantly differently from others, training data might not contain enough variants of the users plans to create a general model that captures as many ways of performing the task as possible. \sidenoteMj{revisar hasta el final del párrafo}On the other hand, reasoning without enough abstraction (i.e., low-level reasoning) about user’s actions is not suitable to that end for several reasons. First of all, those systems tend to be more prone to noise from observation layer such as sensor data, video signal, etc. Second, they are usually designed for an specific domain application, discarding the generalisation mechanisms to ease the reusability of the acquired knowledge for other purpose. Moreover, complex activities are only recognisable at certain level of abstraction, thus a high-level reasoning in this regard enhance the capability of the system to offer valuable assistance when a skill-demanding task is being carried out by the user \cite{chen2012sensor}.} %Thus, it becomes necessary an abstract reasoning throughout the user task for providing a reliable supervision and assistance. 
%%%%%%%%%%%%%%

%\sidenoteMj{revisar esta primera frase}

% In this way, the system should be capable not only of recognising the current state of the task, but also potential user's actions and goals. In short, the possible plans that lead the user to complete the task. 

% It is a fact that for an effective supervision, it is needed to know all the different ways that lead the task to success and, in many cases, 

% \sidenoteJose{Zasca, qué cambio. Aquí se introduce para motivar o para explicar. Si es para explicar, deberíamos empezar con una pregunta, ¿cómo podemos integrar lo mejor de la aproximación basada en conocimiento y la basada en datos? Y aquí supongo que entraría inductive programming.}
% Inductive Programming (IP) \cite{gulwani2015inductive} is a research area where artificial intelligence, machine learning and cognitive science join in order to learn (small) %declarative
% programs from a small set of  examples and some declarative background knowledge. IP provides interesting features that can be highly exploited by the automatic supervision in order to acquire the expert's knowledge. Those systems can be supplied with a start-up knowledge (domain information) and then enriched incrementally by the system through the examples. In this manner, an expert could initially introduce the abstract knowledge, detailing the high-level concepts and task constraints, and then increment it (automatically) by recording some illustrative executions of how this task should be performed. Recently, \cite{monserrat2016knowledge} presented an IP approach that is able to learn automatically the relationships between some high-level activities (defined by the expert) and the observable events detected in video-recorded executions\sidenoteJose{O sea, no hay ya novedad y el problema está resuelto? Habrá que comentar sus limitaciones, no?}. In general, IP approaches rely on declarative languages (i.e., expressed as potentially comprehensible rules) to represent the examples, background knowledge and generalised hypotheses. Thus, the inferred programs can be inspectable and understandable by the domain experts. This would allow experts to monitor these rules and modify those that are not considered appropriate or do not fit the task. Also, declarative languages ease the use of inference mechanisms for logical reasoning (e.g., deduction, induction or abduction). These could be useful for making predictions about the user's behaviour or explaining the system decisions. \sidenoteDavid{¿Pongo alguna propiedad más?¿Cuál?}\sidenoteJose{No, creo que hay de más. Se está alargando mucho. La intro debe tener, problema, idea novedosa y cuatro pinceladas de la solución. Y ya está. Nos falta la idea novedosa, y tenemos trozos de la solución.}\sidenoteDavid{Nuevo}

% \sidenoteJose{Si este párrafo es el que tiene que explicar qué es realmente lo nuevo de este paper, a mí me parece todo generalidades... No va al grano ni del problema ni de la solución.}
% In spite of the possibilities of the IP automated supervisors, there is still a need for approaches that help those systems to bridge the gap between the observed executions from experts, and the logical knowledge acquisition. It is a reality that many contexts of supervision usually have just one correct reference procedure (or at most a few) to compare with, as this requires time and effort from experts. Additionally, some experts can perform the task significantly differently from others, being different plans possible on task accomplishment. Therefore, some kind of generalisation approach will be required to abstract the task structure (i.e., a pattern) from very few demonstrations, and consolidate it in the IP supervisor knowledge base. That means to develop the right mechanisms to put in common the different task observations, mining the dominant pattens, and filter the main steps from the superfluous ones. A refinement mechanism will also be necessary to search, in the space of possible solutions, the most accurate model according to the observed examples. Even when the discrepancies between plans are little or notably.\sidenoteDavid{Nuevo}



%%%%%%%%%%%%%%%%%%% Version MJ %%%%%%%%%%%%%%%
% Inductive Programming (IP) \cite{gulwani2015inductive} is a research area where artificial intelligence, machine learning and cognitive science join together in order to learn (small) declarative programs from a few observations and some declarative background knowledge. IP systems have been also shown successful for the automation of repetitive task in other human-related application domains, such as the FlashFill \cite{gulwani2011automating} and  FlashExtract \cite{gulwani2017framework} tools for data transformation, or the creation of educational content for different subjects (logic, programming or algebra) directly from examples \cite{gulwani2014example}. Needless to say, learning a complex task from a few instances in a physical environment entails many more challenges. However, we believe that this is possible if the training examples are sufficient meaningful for describing the task, an appropriate level of abstraction \sidenoteMj{reasoning?? No entiendo lo siguiente} is achieved, and the right tools and mechanisms are developed to acquire the knowledge of the experts in the matter \cite{monserrat2016knowledge}. But there is also still to bridge the gap between the observed information and the logical knowledge acquisition. Therefore, some kind of generalisation approach is required to that end; that is, put in common the different task observations, mining the dominant plans, and filter the main steps from the superfluous ones. In this regard, a refinement mechanism will also be necessary to search, in the space of possible solutions, the most accurate model according to the observed examples, even when they present little discrepancies between them, or notably different plans of performing the task.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%This challenge has characterised at length the research area of Inductive Programming (IP) \cite{gulwani2015inductive}, area where artificial intelligence, machine learning and cognitive science join together in order to learn human routines, in the form of computer programs, from several examples observations and some declarative background knowledge. IP is concerned about making expert systems learn programs automatically in situations where data become scarce. Moreover, experts knowledge can enhance significantly the system performance by introducing the domain constraints, as long as that knowledge is captured appropriately by the system. Inductive programming has been successful for repetitive task automation in other human-related application domains, such as data transformation tasks with FlashFill \cite{gulwani2011automating} or  FlashExtract \cite{gulwani2017framework} tools, or creating educational content for different subjects as logic, programming or algebra, directly from examples \cite{gulwani2014example}. Needless to say, learning a complex task from a few instances in a physical environment entails many more challenges, however, we believe this is possible if those examples are meaningful enough describing the task, an appropriate level of abstract reasoning is achieved, and the right tools and mechanisms are developed to acquired the knowledge of the experts in the matter \cite{monserrat2016knowledge}. But there is also still to bridge the gap between the observed information and the logical knowledge acquisition. Therefore, some kind of generalisation approach is required to that end; that is, put in common the different task observations, mining the dominant plans, and filter the main steps from the superfluous ones. In this regard, a refinement mechanism will also be necessary to search, in the space of possible solutions, the most accurate model according to the observed examples, even when they present little discrepancies between them, or notably different plans of performing the task.
% \sidenoteDavid{Corregido. Era un trozo de texto que se me había quedado sin comentar.}\sidenoteMj{No creo que haga falta mencionar ILP, aunque falta conexion con IP. Revisar rl resto de parrafo}\sidenoteJose{No, en la intro no más, por favor :-)}


% by developing inductive refinement techniques to find the most accurate model according to the observed examples in a search space of possible manners candidates. As in Inductive Logic Programming (ILP) 

% Mechanisms to But as in other inductive learning context, a general pattern is underlying the examples and must be present in each relevant observation  inductive refinement techniques to find the an underlying representation and most accurate according to the observed examples.

% , all this in order to synthesise the task in a general representation. In  a first incursion in inductive supervision were achieved, where obtained from some meaningful examples performed by skilled experts on the matter, which lend it to be considered as the correct way that must be followed to perform the task under supervision in the proper way . Nevertheless, 
% Nevertheless, mechanism to deal with  and the search space of possible manners of developing it are sufficiently delimited for the system. In this sense, %Inductive Logic Programming (ILP) \cite{muggleton1994inductive} provides 
% some inductive refinement techniques to find the an underlying representation and most accurate according to the observed examples.

% Even though a task can be performed in different ways, we believe that a general pattern underlies them and must be present in each relevant observation. Therefore, there is still necessary to bridge the gap between the observed information to the logical knowledge acquisition with some kind of generalisation mechanism. In supervision contexts where data is lacking and the supervised task is skill demanding for humans, new methods are required to put in common different observations, mining the dominant ways, and filter the main steps from the superfluous ones.

% On the other hand, existing literature in PR (\cite{yang2007learning}, \cite{yang2005learning}, \cite{blythe2001integrated}, \cite{benson1995inductive}, \cite{wang1995learning}) have shown it is possible to acquire the missing knowledge concerning tasks by learning from plan observations. 
 % Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.   %Therefore, there is the possibility of capturing that essence from several but ``rich'' examples. Nonetheless, in supervision contexts where data is lacking and supervised task is skill demanding for humans, there still necessary to bridge the gap between the observed information to the logical knowledge acquisition with some kind of generalisation mechanism. New methods are therefore required to put in common different observations, mining the dominant ways, and filter the main steps from the superfluous ones. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.   

% \textcolor{blue}{David: Voy a reescribir esta parte. Creo que quedará mejor juntandolo con el párrafo anterior}\\
% In order to address this generalisation challenge, the contribution of this paper is twofold: (1) we present a novel inductive approach\sidenoteJose{No sé lo que es un "inductive approach". Es un machine learning approach? o es un "inductive programming approach"? } to extract the underlying  \FullNamePlanSpaceGraph{s} \textcolor{blue}{[quizá denominarlos como (\ShortNamePlanSpaceGraph) o Plan Space Models (PSM)]}\sidenoteJose{Esto ni se ha motivado ni conectado con nada de lo anterior. Llevamos tres páginas y cuando llegamos a las contribuciones, no sabemos que es un PSM... ni por qué hacen falta. El título va de plan patterns... y no se ha explicado qué es. Y estamos en la página 4!} from a set of labelled human activity sequences until all the examples are covered by at least one of those patterns. As an outcome, we get multiple ``compact'' \footnote{we use this term in this paper to mean a smaller size compared to the addition of individuals}\sidenoteDavid{¿Entonces dónde indico esto? Me parece interesante aclarar este concepto.}\sidenoteMj{la footnote no se entiende y ya antes se ha mencionado compacteness} plan patterns, where the main activities and their relationships are kept on it. This allows us to filter the superfluous information that is not strictly necessary to learn the task; (2) we study the coverage of those models according to new instances unseen by those patterns. For this purpose, we use several state-of-the-art metrics from graph theory domain to measure the similarities between a \ShortNamePlanSpaceGraph{} and a given plan %graph 
% instance. All this will be enable us to take a further step towards a real automation of the learning phase\sidenoteJose{automation of the learning phase? Eran los otros métodos manuales?} along the supervision process. Furthermore, our approach makes it possible to deal with the lack of examples and the divergence of ways to perform a skill-demanding\sidenoteJose{skill-demanding?} task. The potentiality of this method will be tested in one domain characterised by the prior handicaps\sidenoteJose{prior handicaps? No entiendo.}: the automatic skill supervision in surgical training tasks. 

% •	Recognise sequences of gestures that are new to the system.
% •	Recognise repetitions.
% •	Detect boundaries of a task.
% •	Identify the optimal representation for a certain task.

% How to get the general planning of a task through a few example sequences?
% How to avoid/reduce the noisy transition between actions of the sequences?

The rest of this paper is organised in the following manner. Section 2 reviews the literature regarding with the automatic supervision and plan recognition. Section 3 presents our method of generalisation using the study case of a typical suturing task. Then, Section 4 presents the experimental setup and results about the application of our generalisation method with a set of real examples of this suturing task. In Section 5 we discuss the experiment results and our method strengths and limitations. Finally, Section 6 depicts our conclusions and further research directions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Párrafo para 
% In literature exists a considerable number of approaches for modelling human plans. 

%Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.  

% in the transition from the detected information to the logical knowledge acquisition in AR is still necessary to design mechanisms, not only to provide the task boundaries, but also to identify an optimal representation of them. Therefore, generalisation methods are required to join the different executions, mining the dominant ways, and filter the main steps from the superfluous ones. This would provide a good initial guess about which activities, together with their relationships, compound the route map where the task steps must flow to fulfil it. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.  Then, given the fact the task is known, the following step is to identify and learn the patterns of correct ways (i.e., the form of the plans) that could achieve the task goal. Nevertheless, the huge challenge here is addressing this objective in contexts where data is lacking. the task is skill demanding and there are multiple forms to perform it. New methods are required to join the different executions, mining the dominant ways, and filter the main steps from the superfluous ones. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.  

% In this way, graph analysis provides multiple features to extract meaningful information from connected structures such a sequence of steps does. Thus, some noteworthy fields such as bioinformatics [ref], social-network analysis [ref], computer vision [ref] and image processing [ref] have taken advantage of these capabilities. Subgraph finding, for instance, enables us to discover recurrent patterns that are hidden in a set of graphs [ref]. In turn, graph comparison is used to group similar graphs into clusters applying a similarity criterion [ref]. Despite the fact that these features are powerful, they are computationally expensive, as the size of the graph grows (NP-hard). Many researches during last decade have provided a wide range of kernels to address this problem.
   
%\textcolor{red}{FALTARÍA ESPECIFICAR EN QUÉ PARTE SE VA A CENTRAR EL ARTÍCULO. Nos vamos a centrar en la parte de aprendizaje y, en concreto, la parte de "aprender" todas las formas de realizar una tarea de forma correcta a partir de unos pocos ejemplos introducidos por los expertos. Además, habría que resaltar que el método de aprendizaje no estaría limitado a la fase de entrenamiento sino que se podría seguir durante toda la vida útil del sistema mientras le sigan llegando ejecucciones correctas llevadas a cabo por el sistema. Además, el aprender todas las formas de realizar correctamente una tarea también es algo que diferencia nuestro sistema de uno de automatización de tareas. En la automatización basta con aprender como ejecutar una tarea correctamente. Además, precisa de aprender todos los detalles de esa tarea. En Supervisión, hay que aprender todas las formas de llevar a cabo una tarea pero no hace falta aprender el detalle, basta con aprender los pasos clave para conseguir llevar a cabo la tarea con éxito. El aprender todas las formas de realizar la tarea y diferenciar entre los pasos clave y los superfluos son los objetivos del trabajo que se presenta en este paper.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/old_introductions/introduction_v9.tex <==
\section{Introduction v9} 

%In this paper, we propose a new method based on Process Mining and Inductive Programming to learn process models for posterior applications in automatic supervision systems. 
Nowadays, there are multiple fields of research that are investigating automatic systems that monitor, recognise and respond to human behaviours, such as Ambient Intelligent \citep{camacho2014ontology} And Context-aware systems \citep{hong2009context}, Advanced Driving Assistants \citep{vskrjanc2018evolving} or Surveillance systems \citep{kardas2017svas} \citep{mabrouk2018abnormal}. In fact, the potential of an automatic supervision system of monotonous and/or complex human processes could be a reasonable alternative to their automation, making the human performance more reliable and efficient because of the constant monitoring at a considerably reduced cost. This supervision would care about whether the operators would be developing the process correctly, detecting deviations from the established models of the process, and advising them in real-time because deviations of the model or by suggesting activities to accomplish the goals of the process (meaningful feedback). As a result, an automatic supervisor could prevent some processes from suboptimal results or implying a potential risk due to human mistakes \citep{birkmeyer2013surgical}. 

In order to do all this, the supervision system need to learn the essence of how one process should be done, coded by a programmer or learnt automatically from examples and procedures provided by experts. Manual coding is time-consuming, rigid and prone to obsolescence. Besides, it requires a big effort to define, or in the extreme case, to directly program all the possible models of performing a process, as well as updating them when new models appear over time. On the other hand, a real automatic supervisor must be general, transversal and pervasive enough to be tuned to multiple domains. Moreover, the number of available examples is often limited, but still the system must learn the different ways in which a process can be performed toward carry out correct supervision. 

Traditionally, similar learning processes have been addressed in Activity Recognition (AR) \citep{sukthankar2014plan}, using both data-based approaches and knowledge-based approaches \citep{chen2012sensor}. To date, data-based approaches have been the predominant way to generalise task models, relying on intensive use of pre-existent data from users’ activities. However, these approaches are not suitable for domains where there is not enough data. Besides, in some cases, it is necessary to define the structure of the task to be learnt previously \citep{hoey2010automated}. An alternative way (i.e., knowledge-based approaches) implies to take advantage of the previous knowledge (bias) about the domain as a resource to generalise or learn a procedure. For example, logic-based approaches obtain semantically clear and compact models, but have problems adapting to different users’ activity habits and handling examples with noise (i.e., infrequent behaviours).

In this paper, we aim to provide a generalisation method to automate the extraction of the essential workflows (i.e., process models) from a few expert executions. Our method overcomes the limitations of the data-based (i.e., learn from a few examples) and knowledge-based approaches (i.e., different behaviours, different models), by using a method based on process mining techniques \citep{van2016process}, Inductive Programming and graph theory. As a result, we obtain models in the form of dependency graphs (\citep{van2004workflow}, \citep{yan2005mining}, \citep{carrington2005models}, \citep {papadimitriou2010web}), typical representation for process models where the model nodes represent the involved activities, and the directed arcs represent the order relation between these activities. These models have two advantages: they are easily understandable and make it possible to filter the non-essential activities \citep{van2016process}. One activity is considered non-essential if its execution is not necessary to finish the process correctly. The algorithm also ensures the validity of each model, as a complete representation of the process, and the feasibility of it by checking that, at least, one training example is covered by the output model. Finally, we have analysed the generalisation, simplicity and fitting properties of the resulting models. As far as we know this is the first approach that proposes the combination of dependency graphs and an inductive method for process modelling in a knowledge-based supervision system. To analyse the applicability of the model, we have tested the potentiality of this method in a very challenging environment that considers all the mentioned requirements: the automatic skill supervision in surgical training tasks.

The rest of this paper is organised in the following manner. Section \ref{motivation} presents briefly the motivation of this work. In this section we want to answer the question of why we have developed this research. Section \ref{matandmet} presents our mining approach based on dependency graphs. Then, Section \ref{s:results} presents the experimental setup and the results of applying our approach with a set of real examples of a surgical exercises. In Section \ref{s:discussion} we discuss the experimental results and the strengths and limitations of our method. Section \ref{background} reviews the literature on automatic supervision and process modelling. Finally, Section \ref{s:conclusions} outlines our conclusions and further research directions.

%%%%%%%%%%%% Versión antigua con Comentarios Jose %%%%%%%%%%%%

% Today, there are many human tasks whose automation is not possible yet, despite being repetitive. The automatic supervision of these tasks has arisen as a suitable step for making them more reliable and efficient, in the interim of making them fully automated. Also, supervision and overseeing may be key for contexts where other automated systems are being used, but still not very reliable. 
% %Despite the human interaction is still indispensable to perform such tasks, a  system could assist the human in the development of the task. In this sense, that system, as 
% An automated supervisor would be able to monitor whether operators are performing the task correctly, detect deviations from the established plans, and advice them in real time %, if that were the case, 
% with meaningful feedback. \sidenoteJose{A partir de aqui se repite lo mismo una y otra vez. Reescribo}Automated supervision could have a significant effect on two important spheres. On one hand, some tasks may be easily spoilt, may lead to suboptimal results or imply a potential risk by a human mistake. The supervisor system could trace the operator activities and spot the deviations from the expected performance, %. The same applies to those jobs subject to pre-established 
% workflow or protocol. %, where automated supervision would make it more secure. 
% On the other hand, humans learn some tasks more efficiently if they have continuous supervision and get meaningful feedback, but this overseeing (from an expert or a teacher) is usually expensive. Hence, the acquisition of new skills in training environments would be enhanced through systems performing automated supervision and useful feedback. Indeed, poor technical skills have been associated with adverse outcomes or even tragic consequences \cite{birkmeyer2013surgical}. These two stages (training and operation) are directly connected. The better training is through intensive monitoring and feedback the less prone to errors the operators will be. This has been shown % at is why in some domains such as surgery, it is foreseen that those systems can be potentially beneficial to improve the  
% in surgical/interventional care \cite{vedula2017surgical}.  \sidenoteJose{De nuevo nos repetimos un montón en lo que queda.} In some educational contexts, the traditional model of teaching skills relies on supervision and demonstration by experts in the matter.This method has traditionally suffered important limitations, such as limited access to realistic test beds or the availability of experts’ time to give immediate feedback and guidance during each exercise. Automatic supervisors, as coaching systems, would be an alternative to enable inexperienced trainees to learn without a continuous human expert supervision. Previously, these systems should assimilate the experts knowledge in order to provide an effective assistance and supervision. \sidenoteDavid{Nuevo}

%%%%%%%%%%%%%%%%%
% Version antigua
%%%%%%%%%%%%%%%%%
% \textcolor{blue}{Despite humans are still indispensable to develop complex tasks whose automation is not feasible yet, supervision systems have arisen as a suitable alternative to automatically assist humans when they are performing those tasks.} \sidenoteDavid{Lo he reescrito, ¿mejor así?}\sidenoteMj{rehacer la frase siguiente}In contexts where an appropriate use of abstract knowledge or an interaction capability with the surrounding environment are required by an operator or apprentice, those systems may be able to supervise whether a human is performing the task correctly, detect deviations from the established plan, and advice him or her in real time if that were the case. The training of new skills and the human errors during their execution could entail a high cost that could be reduced by automated supervision systems indicating when, where and how a protocol error takes place, in a comprehensible way for the user or the professional. \textcolor{blue}{This technology is specially applicable to supervise jobs under a well-defined workflow or strict protocol, or also for training environments where a continuous monitoring and feedback is the basis for a correct learning of procedures.}\sidenoteDavid{He usado esta frase del Explora. Creo que explica mejor la motivación de la supervisión automática} \sidenoteMj{rehacer la frase siguiente}Namely, it could be seen as an automatic expert in the matter made to help in this task and ultimately to enhance itself by supervision and guidance. These systems has been strengthen (mainly) by advances in the Activity Recognition (AR) field \cite{sukthankar2014plan}, which have provided with a wide range of approaches to recognise human activities in multiple domains, such as industry (\cite{marinho2017preliminary}, \cite{maekawa2016toward}%, \cite{roitberg2015multimodal}, \cite{wu2012automated}, \cite{petrovic2010context}
% ),  surveillance (\cite{batchuluun2017fuzzy}, \cite{kardas2017svas}, \cite{mabrouk2017abnormal}%, \cite{hu2013incremental}, \cite{zin2010markov}, \cite{ran2010applications}
% ), smart environments and daily-living assistance (\cite{chernbumroong2013elderly}, \cite{banos2012daily}, \cite{hoey2010automated}%\cite{ayase2008method}, \cite{camacho2014ontology}, \cite{brdiczka2009learning},  \cite{yordanova2017s}
% ), or medicine and health-care (\cite{sanchez2008activity}, \cite{corchado2010using}, \cite{negin2018praxis}%, \cite{nakawala2017development}, \cite{soutschek_measurement_2010}, \cite{hein_saphire_nodate}, \cite{dosis2005synchronized}, \cite{ghali2003object}, \cite{yordanova2017situation}
% ). The socioeconomic impact derived from automatic supervision %the latter 
% would be remarkable for many human daily situations, allowing the instant detection of a human mistake at work that can cause a risky situation, or assisting people during their task accomplishment by providing meaningful and comprehensible feedback. 

% Automatic supervisors usually work in two sequential phases. Firstly, the systems must learn the essence of how one task should be done (i.e., a model of the task), coded by a programmer or learnt from examples and procedures provided by experts. Secondly, once the different ways of performing a task have been learnt, the system should be able to supervise the task when it is performed by a user. As the user operates, the system will compare the ongoing actions with the generalised model and will spot the discrepancies and possible amendments in real time. Considering that there may be different ways of correcting a possible wrong action, the system must be able to generalise in such a way that goes beyond particular cases and `understand' the intermediate goals of a task.\sidenoteJose{Rewritten}
%learn all of them (\sidenoteMj{lo del parentesis lo he añadido yo}or at least the most extensively used)\sidenoteDavid{Ok} to perform a proper supervision.

% The extraction of a computational task model, in a way that allows a system to conduct supervision, is a topic widely addressed in the area of Activity Recognition (AR). Applications of AR have been proposed 
% for a wide range of domains, such as industry (\cite{marinho2017preliminary}, \cite{maekawa2016toward}%, \cite{roitberg2015multimodal}, \cite{wu2012automated}, \cite{petrovic2010context}
% ),  surveillance (\cite{batchuluun2017fuzzy}, \cite{kardas2017svas}, \cite{mabrouk2017abnormal}%, \cite{hu2013incremental}, \cite{zin2010markov}, \cite{ran2010applications}
%  ), smart environments and daily-living assistance (\cite{chernbumroong2013elderly}, \cite{banos2012daily}, \cite{hoey2010automated}%\cite{ayase2008method},  \cite{brdiczka2009learning},  \cite{yordanova2017s}, \cite{camacho2014ontology}
%  ), or medicine and health-care (\cite{sanchez2008activity}, \cite{corchado2010using}, \cite{negin2018praxis}). All these applications have been motivated (mainly) by the objective of allowing computing systems to  assist humans with their tasks. 
%  \sidenoteDavid{Nuevo}\sidenoteJose{Es Activity Recognition lo mismo que Automatic Supervision? Este párrafo da a entender que sí, y tira por tierra toda la novedad que podría tener el artículo en cuanto a supervisión, y los primeros párrafos. Para mí, activity recognition es parecido pero no lo mismo. Igual estoy equivocado, pero los nombres, al menos, son muy diferentes.}
 
 %, \cite{nakawala2017development}, \cite{soutschek_measurement_2010}, \cite{hein_saphire_nodate}, \cite{dosis2005synchronized}, \cite{ghali2003object}, \cite{yordanova2017situation}
%

% \sidenoteMj{Hasta el final de este párrafo hay que revisarlo}\sidenoteDavid{La he retocado, no sé si está más clara ahora.}\textcolor{blue}{In this way, the system should be capable not only of recognising the current state of the task, but also potential user's actions and goals. In short, the possible plans that lead the user to complete the task. In this context, Plan Recognition (PR) \cite{sukthankar2014plan} plays a fundamental role in the learning phase (the first one mentioned before) in order to generalise the execution of a given task.}


%%%%%%%%%%%% Version anterior %%%%%%%%%%%%

% These automatic supervisors usually work in two sequential phases. Firstly, the systems must learn the essence of how one task should be done (i.e. a pattern) from the examples provided by experts. Secondly, once the different ways of performing a task have been learnt, the system should be able to supervise the task executed by an apprentice by comparing her execution with the patterns learnt in the first phase. Therefore, considering that there may be different ways of correctly executing one task, the system must be able to learn all of them (\sidenoteMj{lo del parentesis lo he añadido yo}or at least the most extensively used)\sidenoteDavid{Ok} to perform a proper supervision. 
% %Therefore, considering that there may be different ways of correctly executing one task, the system must learn all of them to perform a proper supervision.
% \sidenoteMj{Hasta el final de este párrafo hay que revisarlo}\sidenoteDavid{La he retocado, no sé si está más clara ahora.}\textcolor{blue}{In this way, the system should be capable not only of recognising the current state of the task, but also potential user's actions and goals. In short, the possible plans that lead the user to complete the task. In this context, Plan Recognition (PR) \cite{sukthankar2014plan} plays a fundamental role in the learning phase (the first one mentioned before) in order to generalise the execution of a given task.}
%%%%%%%%%%%%


% ref para el párrafo\cite{chen2012sensor}

% \sidenoteJose{La intro no debería pasar de dos páginas y por fin parece que llegamos a la motivación del paper.}\sidenoteJose{Y párrafos de casi una página. Son infumables. Hay que ir al grano, sintetizar y trocear}
% According to the mechanism that is used during the learning phase, the AR approaches can be distinguished in data-based approaches and knowledge-based approaches \cite{chen2012sensor}. Traditionally, the AR applications have been dominated by the first one. These rely on an intensive use of preexistent data of users’ behaviours to obtain the task model. Data mining and machine learning techniques are used to create probabilistic or statistical models. % that are trained in a subsequent step. 
% Although both techniques are undoubtedly contrasted\sidenoteJose{lo de contrasted no creo que funcione en inglés. En cualquier caso, si funcionan no se motiva la segunda parte de la frase. ¿Tienen limitaciones, sí o no?}, the automatic supervision must go away from these methods\sidenoteJose{go away? rewrite...} if the supervision is expected to be general, transversal and pervasive enough to be tuned to multiple domains. This is motivated by several reasons. Firstly, many domains that could potentially  be benefitted by automated supervisors, are characterised by very little or sparse activity data. Although there are plenty of datasets about human activities \cite{chaquet2013survey}, this data becomes useless when the set of activities required to learn a task is specific to certain domain\sidenoteJose{No entiendo esta frase, me parece un poco contradictoria}. As a result, new data must be recorded and annotated. This process is costly and time consuming. Hence, supervision systems must learn from fewer supervised reference procedures to generalise the task. Secondly, the information necessary to make automatic supervision effective enough is not only in the observations. Tasks are more than a simple sequence of low-level actions. Indeed, they become intelligible to humans when certain level of abstraction is reached. The system should allow the definition of %deep concepts and 
% abstract knowledge in order to capture the intention and meaning of the user's actions. %ongoing performance of the user. 
% Moreover, assertive supervisors must go a step further than simple user's action recognition.\sidenoteJose{Aha... primera diferencia entre supervisor y recogniser... Pero llega muy tarde y de refilón} Deviation detection and proper feedback providing must be overhauled.\sidenoteJose{Frase no gramatical} Therefore, learning process\sidenoteJose{Learning o supervision? De todas maneras este desiderata suena a carta a los reyes} must become more cognitive and predictable, by taking more advantages of intentions, constraints, source and context of the data, rather than just looking at information as raw data. Finally, when only few observations are available, it becomes even more important to take advantage of the rich knowledge that domain experts can provide to the virtual supervisor.\sidenoteJose{Esto no se ha dicho ya? Este párrafo no acaba nunca} Appropriate learning mechanisms to acquire, codify and make use of the experts knowledge will be basis to that end.\sidenoteJose{Frase vacía} Alternatively to a data-driven approach, a knowledge-based approach makes use of those mechanisms to capture the prior knowledge in the domain to generalise the procedure to supervise.\sidenoteJose{De nuevo, esto no se ha dicho ya?} In those application domains, where automatic supervision must learn from a few reference procedures, the appropriate technology must be chosen to learn a model from incomplete information.\sidenoteJose{Frase vacía.} For that reason, an inductive approach\sidenoteJose{Qué es un "inductive approach", para mí es sinónimo de "learnign"} would be more suitable in order to fill those gaps by making the most of experts' experience and background. \sidenoteJose{En resumen, si queremos decir que nuestra propuesta recoge lo mejor de los dos mundos y consigue abstraer porque usa X, Y y Z, en vez de W, R y S no ha quedado nada claro.}
% \sidenoteDavid{Nuevo}

%%%%%%%%%%%%%%%%%
% Version antigua
%%%%%%%%%%%%%%%%%
% In those context in which the supervision system must learn from one correct reference procedure (or at most a few), automatic supervision must go away from classical machine learning and statistical modelling and use some other methods that allow the introduction of strong bias that is represented by the prior knowledge about the domain and environment.
% Though, nowadays, there are datasets with many human activities in different situations and scenarios to generate those model \cite{chaquet2013survey}, certain domain activities are so specialised that new data must be recorded and annotated. This is costly and timeconsuming. Additionally, it is a fact that people can perform certain activities significantly differently from others. Training data might not contain enough variants of the users plans to create a general model capable of expressing as many ways of performing the task as possible. This usually leads to models that are not scalable or reusable. Finally, supervising a task involves much more than a sequence of linked activities that can be derived from the data. Low-level actions makes it difficult to capture the intention and meaning of the ongoing performance of the user. 
% textcolor{red}{and a short-sighted reasoning  \sidenoteMj{la palabra reasoning tiene que explicarse. Te refieres a que los patrones no tienen en cuenta las acciones ni la tarea?} in regard to the actor's actions and the ongoing task. On one hand, most recognition algorithms require extensive amounts of training data. \sidenoteMj{las 2 frases que vienen a continuacion no se entienden}
% Although there are multiple datasets based on human activities for different situations and scenarios \cite{chaquet2013survey}, when certain tasks to be monitored entail a set of very specific activities, make the previous dataset useless to train a model for that purpose. Therefore, new data must be gathered and annotated, with the subsequent economic and time-consuming effort which it implies. Additionally, as in some human routines some people can perform certain activities significantly differently from others, training data might not contain enough variants of the users plans to create a general model that captures as many ways of performing the task as possible. \sidenoteMj{revisar hasta el final del párrafo}On the other hand, reasoning without enough abstraction (i.e., low-level reasoning) about user’s actions is not suitable to that end for several reasons. First of all, those systems tend to be more prone to noise from observation layer such as sensor data, video signal, etc. Second, they are usually designed for an specific domain application, discarding the generalisation mechanisms to ease the reusability of the acquired knowledge for other purpose. Moreover, complex activities are only recognisable at certain level of abstraction, thus a high-level reasoning in this regard enhance the capability of the system to offer valuable assistance when a skill-demanding task is being carried out by the user \cite{chen2012sensor}.} %Thus, it becomes necessary an abstract reasoning throughout the user task for providing a reliable supervision and assistance. 
%%%%%%%%%%%%%%

%\sidenoteMj{revisar esta primera frase}

% In this way, the system should be capable not only of recognising the current state of the task, but also potential user's actions and goals. In short, the possible plans that lead the user to complete the task. 

% It is a fact that for an effective supervision, it is needed to know all the different ways that lead the task to success and, in many cases, 

% \sidenoteJose{Zasca, qué cambio. Aquí se introduce para motivar o para explicar. Si es para explicar, deberíamos empezar con una pregunta, ¿cómo podemos integrar lo mejor de la aproximación basada en conocimiento y la basada en datos? Y aquí supongo que entraría inductive programming.}
% Inductive Programming (IP) \cite{gulwani2015inductive} is a research area where artificial intelligence, machine learning and cognitive science join in order to learn (small) %declarative
% programs from a small set of  examples and some declarative background knowledge. IP provides interesting features that can be highly exploited by the automatic supervision in order to acquire the expert's knowledge. Those systems can be supplied with a start-up knowledge (domain information) and then enriched incrementally by the system through the examples. In this manner, an expert could initially introduce the abstract knowledge, detailing the high-level concepts and task constraints, and then increment it (automatically) by recording some illustrative executions of how this task should be performed. Recently, \cite{monserrat2016knowledge} presented an IP approach that is able to learn automatically the relationships between some high-level activities (defined by the expert) and the observable events detected in video-recorded executions\sidenoteJose{O sea, no hay ya novedad y el problema está resuelto? Habrá que comentar sus limitaciones, no?}. In general, IP approaches rely on declarative languages (i.e., expressed as potentially comprehensible rules) to represent the examples, background knowledge and generalised hypotheses. Thus, the inferred programs can be inspectable and understandable by the domain experts. This would allow experts to monitor these rules and modify those that are not considered appropriate or do not fit the task. Also, declarative languages ease the use of inference mechanisms for logical reasoning (e.g., deduction, induction or abduction). These could be useful for making predictions about the user's behaviour or explaining the system decisions. \sidenoteDavid{¿Pongo alguna propiedad más?¿Cuál?}\sidenoteJose{No, creo que hay de más. Se está alargando mucho. La intro debe tener, problema, idea novedosa y cuatro pinceladas de la solución. Y ya está. Nos falta la idea novedosa, y tenemos trozos de la solución.}\sidenoteDavid{Nuevo}

% \sidenoteJose{Si este párrafo es el que tiene que explicar qué es realmente lo nuevo de este paper, a mí me parece todo generalidades... No va al grano ni del problema ni de la solución.}
% In spite of the possibilities of the IP automated supervisors, there is still a need for approaches that help those systems to bridge the gap between the observed executions from experts, and the logical knowledge acquisition. It is a reality that many contexts of supervision usually have just one correct reference procedure (or at most a few) to compare with, as this requires time and effort from experts. Additionally, some experts can perform the task significantly differently from others, being different plans possible on task accomplishment. Therefore, some kind of generalisation approach will be required to abstract the task structure (i.e., a pattern) from very few demonstrations, and consolidate it in the IP supervisor knowledge base. That means to develop the right mechanisms to put in common the different task observations, mining the dominant pattens, and filter the main steps from the superfluous ones. A refinement mechanism will also be necessary to search, in the space of possible solutions, the most accurate model according to the observed examples. Even when the discrepancies between plans are little or notably.\sidenoteDavid{Nuevo}



%%%%%%%%%%%%%%%%%%% Version MJ %%%%%%%%%%%%%%%
% Inductive Programming (IP) \cite{gulwani2015inductive} is a research area where artificial intelligence, machine learning and cognitive science join together in order to learn (small) declarative programs from a few observations and some declarative background knowledge. IP systems have been also shown successful for the automation of repetitive task in other human-related application domains, such as the FlashFill \cite{gulwani2011automating} and  FlashExtract \cite{gulwani2017framework} tools for data transformation, or the creation of educational content for different subjects (logic, programming or algebra) directly from examples \cite{gulwani2014example}. Needless to say, learning a complex task from a few instances in a physical environment entails many more challenges. However, we believe that this is possible if the training examples are sufficient meaningful for describing the task, an appropriate level of abstraction \sidenoteMj{reasoning?? No entiendo lo siguiente} is achieved, and the right tools and mechanisms are developed to acquire the knowledge of the experts in the matter \cite{monserrat2016knowledge}. But there is also still to bridge the gap between the observed information and the logical knowledge acquisition. Therefore, some kind of generalisation approach is required to that end; that is, put in common the different task observations, mining the dominant plans, and filter the main steps from the superfluous ones. In this regard, a refinement mechanism will also be necessary to search, in the space of possible solutions, the most accurate model according to the observed examples, even when they present little discrepancies between them, or notably different plans of performing the task.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%This challenge has characterised at length the research area of Inductive Programming (IP) \cite{gulwani2015inductive}, area where artificial intelligence, machine learning and cognitive science join together in order to learn human routines, in the form of computer programs, from several examples observations and some declarative background knowledge. IP is concerned about making expert systems learn programs automatically in situations where data become scarce. Moreover, experts knowledge can enhance significantly the system performance by introducing the domain constraints, as long as that knowledge is captured appropriately by the system. Inductive programming has been successful for repetitive task automation in other human-related application domains, such as data transformation tasks with FlashFill \cite{gulwani2011automating} or  FlashExtract \cite{gulwani2017framework} tools, or creating educational content for different subjects as logic, programming or algebra, directly from examples \cite{gulwani2014example}. Needless to say, learning a complex task from a few instances in a physical environment entails many more challenges, however, we believe this is possible if those examples are meaningful enough describing the task, an appropriate level of abstract reasoning is achieved, and the right tools and mechanisms are developed to acquired the knowledge of the experts in the matter \cite{monserrat2016knowledge}. But there is also still to bridge the gap between the observed information and the logical knowledge acquisition. Therefore, some kind of generalisation approach is required to that end; that is, put in common the different task observations, mining the dominant plans, and filter the main steps from the superfluous ones. In this regard, a refinement mechanism will also be necessary to search, in the space of possible solutions, the most accurate model according to the observed examples, even when they present little discrepancies between them, or notably different plans of performing the task.
% \sidenoteDavid{Corregido. Era un trozo de texto que se me había quedado sin comentar.}\sidenoteMj{No creo que haga falta mencionar ILP, aunque falta conexion con IP. Revisar rl resto de parrafo}\sidenoteJose{No, en la intro no más, por favor :-)}


% by developing inductive refinement techniques to find the most accurate model according to the observed examples in a search space of possible manners candidates. As in Inductive Logic Programming (ILP) 

% Mechanisms to But as in other inductive learning context, a general pattern is underlying the examples and must be present in each relevant observation  inductive refinement techniques to find the an underlying representation and most accurate according to the observed examples.

% , all this in order to synthesise the task in a general representation. In  a first incursion in inductive supervision were achieved, where obtained from some meaningful examples performed by skilled experts on the matter, which lend it to be considered as the correct way that must be followed to perform the task under supervision in the proper way . Nevertheless, 
% Nevertheless, mechanism to deal with  and the search space of possible manners of developing it are sufficiently delimited for the system. In this sense, %Inductive Logic Programming (ILP) \cite{muggleton1994inductive} provides 
% some inductive refinement techniques to find the an underlying representation and most accurate according to the observed examples.

% Even though a task can be performed in different ways, we believe that a general pattern underlies them and must be present in each relevant observation. Therefore, there is still necessary to bridge the gap between the observed information to the logical knowledge acquisition with some kind of generalisation mechanism. In supervision contexts where data is lacking and the supervised task is skill demanding for humans, new methods are required to put in common different observations, mining the dominant ways, and filter the main steps from the superfluous ones.

% On the other hand, existing literature in PR (\cite{yang2007learning}, \cite{yang2005learning}, \cite{blythe2001integrated}, \cite{benson1995inductive}, \cite{wang1995learning}) have shown it is possible to acquire the missing knowledge concerning tasks by learning from plan observations. 
 % Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.   %Therefore, there is the possibility of capturing that essence from several but ``rich'' examples. Nonetheless, in supervision contexts where data is lacking and supervised task is skill demanding for humans, there still necessary to bridge the gap between the observed information to the logical knowledge acquisition with some kind of generalisation mechanism. New methods are therefore required to put in common different observations, mining the dominant ways, and filter the main steps from the superfluous ones. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.   

% \textcolor{blue}{David: Voy a reescribir esta parte. Creo que quedará mejor juntandolo con el párrafo anterior}\\
% In order to address this generalisation challenge, the contribution of this paper is twofold: (1) we present a novel inductive approach\sidenoteJose{No sé lo que es un "inductive approach". Es un machine learning approach? o es un "inductive programming approach"? } to extract the underlying  \FullNamePlanSpaceGraph{s} \textcolor{blue}{[quizá denominarlos como (\ShortNamePlanSpaceGraph) o Plan Space Models (PSM)]}\sidenoteJose{Esto ni se ha motivado ni conectado con nada de lo anterior. Llevamos tres páginas y cuando llegamos a las contribuciones, no sabemos que es un PSM... ni por qué hacen falta. El título va de plan patterns... y no se ha explicado qué es. Y estamos en la página 4!} from a set of labelled human activity sequences until all the examples are covered by at least one of those patterns. As an outcome, we get multiple ``compact'' \footnote{we use this term in this paper to mean a smaller size compared to the addition of individuals}\sidenoteDavid{¿Entonces dónde indico esto? Me parece interesante aclarar este concepto.}\sidenoteMj{la footnote no se entiende y ya antes se ha mencionado compacteness} plan patterns, where the main activities and their relationships are kept on it. This allows us to filter the superfluous information that is not strictly necessary to learn the task; (2) we study the coverage of those models according to new instances unseen by those patterns. For this purpose, we use several state-of-the-art metrics from graph theory domain to measure the similarities between a \ShortNamePlanSpaceGraph{} and a given plan %graph 
% instance. All this will be enable us to take a further step towards a real automation of the learning phase\sidenoteJose{automation of the learning phase? Eran los otros métodos manuales?} along the supervision process. Furthermore, our approach makes it possible to deal with the lack of examples and the divergence of ways to perform a skill-demanding\sidenoteJose{skill-demanding?} task. The potentiality of this method will be tested in one domain characterised by the prior handicaps\sidenoteJose{prior handicaps? No entiendo.}: the automatic skill supervision in surgical training tasks. 

% •	Recognise sequences of gestures that are new to the system.
% •	Recognise repetitions.
% •	Detect boundaries of a task.
% •	Identify the optimal representation for a certain task.

% How to get the general planning of a task through a few example sequences?
% How to avoid/reduce the noisy transition between actions of the sequences?


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Párrafo para 
% In literature exists a considerable number of approaches for modelling human plans. 

%Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.  

% in the transition from the detected information to the logical knowledge acquisition in AR is still necessary to design mechanisms, not only to provide the task boundaries, but also to identify an optimal representation of them. Therefore, generalisation methods are required to join the different executions, mining the dominant ways, and filter the main steps from the superfluous ones. This would provide a good initial guess about which activities, together with their relationships, compound the route map where the task steps must flow to fulfil it. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.  Then, given the fact the task is known, the following step is to identify and learn the patterns of correct ways (i.e., the form of the plans) that could achieve the task goal. Nevertheless, the huge challenge here is addressing this objective in contexts where data is lacking. the task is skill demanding and there are multiple forms to perform it. New methods are required to join the different executions, mining the dominant ways, and filter the main steps from the superfluous ones. Only in this way, it will be provided both the key steps and the diversity of performing forms to the system.  

% In this way, graph analysis provides multiple features to extract meaningful information from connected structures such a sequence of steps does. Thus, some noteworthy fields such as bioinformatics [ref], social-network analysis [ref], computer vision [ref] and image processing [ref] have taken advantage of these capabilities. Subgraph finding, for instance, enables us to discover recurrent patterns that are hidden in a set of graphs [ref]. In turn, graph comparison is used to group similar graphs into clusters applying a similarity criterion [ref]. Despite the fact that these features are powerful, they are computationally expensive, as the size of the graph grows (NP-hard). Many researches during last decade have provided a wide range of kernels to address this problem.
   
%\textcolor{red}{FALTARÍA ESPECIFICAR EN QUÉ PARTE SE VA A CENTRAR EL ARTÍCULO. Nos vamos a centrar en la parte de aprendizaje y, en concreto, la parte de "aprender" todas las formas de realizar una tarea de forma correcta a partir de unos pocos ejemplos introducidos por los expertos. Además, habría que resaltar que el método de aprendizaje no estaría limitado a la fase de entrenamiento sino que se podría seguir durante toda la vida útil del sistema mientras le sigan llegando ejecucciones correctas llevadas a cabo por el sistema. Además, el aprender todas las formas de realizar correctamente una tarea también es algo que diferencia nuestro sistema de uno de automatización de tareas. En la automatización basta con aprender como ejecutar una tarea correctamente. Además, precisa de aprender todos los detalles de esa tarea. En Supervisión, hay que aprender todas las formas de llevar a cabo una tarea pero no hace falta aprender el detalle, basta con aprender los pasos clave para conseguir llevar a cabo la tarea con éxito. El aprender todas las formas de realizar la tarea y diferenciar entre los pasos clave y los superfluos son los objetivos del trabajo que se presenta en este paper.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Motivation} \label{motivation}

Learning the process that underlies a human task from the observation of a few correct executions is a complicated challenge for a machine. Something that humans can do naturally and easily, such as identifying what is required to complete a task (i.e, actions, objects, intermediate states) with just a couple of examples, for a machine is a real challenge and very difficult to address when the number of examples is low. Although the steps of the task can be specified and clear, two people can perform sequences of very different activities that meet the specifications. These differences are usually motivated by the small differences in the initial stages in each example, the degree of freedom offered by the task, the previous experience of the person executing it or the interpretation that this makes of the instructions. In this process of generalisation, a human solves in a natural way the points in common and the differences between the observations, creating an abstract scheme of what he needs to be able to perform the task and the ways he could do it. 

How to perform this generalisation in order to make a system learn the task is not trivial for some context. Specifically, if this system has to take decisions to assist people. Let us imagine a scenario where a system has to supervise if a person is cooking right a carrot soup. Table \ref{tbl:cooking_vocabulary} shows the vocabulary of activities that are involved in this task. Previously, the system has observed the following two examples of how to cook this dish (in the form of sequences of activities): ``$SABCDFGHIMOPT$'' and ``$SABCEFGJKLNOPT$''. These examples show two forms of cooking: using a microwave or using the kitchen stove. One could think of a possible generalisation is ``$SABC \{D|E\}FG\{HIM|JKLN\}OPT$'', where ``|'' means a disjunction between two options of activity groups for that section of the task. As can be seen, this generalisation takes both examples as valid, but also other cases that are far for being safe for the person who is cooking. An example would be ``$SABCEFGHIMOPT$'', where the person takes a metal pot to put inside the ingredients and then put the metal pot into the microwave to prepare the soup. The system would give it as a valid sequence following the model above, but these actions are completely contraindicated for the task that is intended. 

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[!t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cl}
\multicolumn{1}{l}{Activity Code} & Activity Description \\ \hline
S & Start the task \\
A & Peel the carrot \\
B & Wash the carrot \\
C & Cut the carrot into pieces \\
D & Take a glass pot \\
E & Take a metal pot \\
F & Fill the pot with water \\
G & Add salt \\
H & Put the pot into the microwave. \\
I & Turn on the microwave to the maximum (15 minutes). \\
J & Put the pot on the stove \\
K & Turn on the stove to the maximum (10 minutes). \\
L & Reduce the stove to the minimum (30 minutes). \\
M & Turn off the microwave. \\
N & Turn off the stove. \\
O & Take a deep dish. \\
P & Add two large spoonful of soups on the dish. \\
T & Finish the task
\end{tabular}%
}
\caption{Vocabulary of activities for cooking a carrot soup. }
\label{tbl:cooking_vocabulary}
\end{table}


Thus, because the lack of negative examples, the solution must be precise as much as possible (being as close as possible to the observed examples), while ensuring the generality that is intended for supervision (determine those key steps for the task and how they are reached by following the previous ones). Therefore, every "generalisation" that is found must be supported by at least one positive execution in order to demonstrate that this generalisation really shows a plausible way to accomplish the task. In addition, there is the possibility of the presence of "non-essential" activities that should be suppressed during the learning / generalisation process of the task.

In summary: the need to learn from few examples, all positive, learning the different ways of executing a task and the possibility of the presence of noise (in the form of non-essential activities) at the same time is a complex task that does not solve the tools currently existing. That is why the need for the developments described in this paper has arisen.


==> sections/sobras_material_methods.tex <==
Once the models %workflows 
have been created, they can be applied to new dependency graphs %(not seen during training)
in order to determine whether they are represented by the models %workflows
\sidenoteJose{Hemos definido esto? Qué significa que un workflow representa un dependency graph? YO creo que no. Aparte en ningún momento hemos definido lo que es un workflow. Un workflow es un dependency graph? No se ha dicho.}. This is a way of knowing how well the models are able to generalise these new examples. %Given the set of new dependency graphs and the set of workflows, we check for each workflow, which examples are overlapped by it.
The models are applied in the order in that they were generated with the purpose of avoiding the inconsistency problem that could arise in the case that one dependency graph overlaps with more than one model\sidenoteJose{Por qué es una inconsistenacia que un ejemplo solape con un workflow? O es que un modelo no es un workflow? Me muero con los mil nombres para la misma cosa.}. %Therefore, when an example is overlapped by a workflow, we annotate the example with an identification label associated with the workflow. Once the example is labelled, we remove the example from the set of dependency graphs. In this sense,
This process can be seen as a classification procedure in that the models are the classes, and each dependency graph is assigned to the label identifying the workflow with which it overlaps\sidenoteJose{No me gusta nada la analogía con "classification"... Más lío. Si se quiere decir que un ejemplo no puede ser cubierto por más de un workflow, eso debe ponerse como definición del problema, un par de páginas antes! Y explicar por qué. Entiendo que la definición del problema, que no se ha hecho, insisto, es que varias maneras de hacer una cosa se entiende como maneras alternativas (y no compatibles). O sea si un ejemplo sigue una forma, no sigue otra. Esto es crucial, y aparece en la página 9 del paper por primera vez!}. %We repeat the above process until we have tested all workflows.
Note that, unlike classification problems, it could be the case that a dependency graph was not represented by any workflow. %In that case, we will have dependency graphs without classifying at the end of this workflow application process.
\sidenoteJose{Mejor quitamos la analogía con classifcation, please...}

\sidenoteMJ{He quitado esta frase. The number of $G_i$ that overlap with $\ThresholdGraph[+]$ is an indicator of the support of $\ThresholdGraph[+]$ in $\mathcal{G}$}

To experimentally evaluate our approach, we implemented a prototype using the programming language R\footnote{https://www.r-project.org/}.
